Gaze into the Pattern: Characterizing Spatial Patterns with Internal Temporal Correlations for Hardware Prefetching

Hardware prefetching is one of the most widely-used techniques for hiding long data access latency. To address the challenges faced by hardware prefetching, architects have proposed to detect and exploit the spatial locality at the granularity of spatial region. When a new region is activated, they try to find similar previously accessed regions for footprint prediction based on system-level environmental features such as the trigger instruction or data address. However, we find that such context-based prediction cannot capture the essential characteristics of access patterns, leading to limited flexibility, practicality and suboptimal prefetching performance. In this paper, inspired by the temporal property of memory accessing, we note that the temporal correlation exhibited within the spatial footprint is a key feature of spatial patterns. To this end, we propose Gaze, a simple and efficient hardware spatial prefetcher that skillfully utilizes footprint-internal temporal correlations to efficiently characterize spatial patterns. Meanwhile, we observe a unique unresolved challenge in utilizing spatial footprints generated by spatial streaming, which exhibit extremely high access density. Therefore, we further enhance Gaze with a dedicated two-stage approach that mitigates the over-prefetching problem commonly encountered in conventional schemes. Our comprehensive and diverse set of experiments show that Gaze can effectively enhance the performance across a wider range of scenarios. Specifically, Gaze improves performance by 5.7\% and 5.4\% at single-core, 11.4\% and 8.8\% at eight-core, compared to most recent low-cost solutions PMP and vBerti.

==> texfile/10_ack.tex <==
\section*{Acknowledgements}
% \vspace{-5pt}
\label{sec:ACKNOWLEDGMENTS}
We thank all the anonymous reviewers, as well as our shepherd, for their valuable comments. 
This work was supported in part by the National Key R\&D Program of China (Grant No. 2023YFB4502902).
% Chentao Wu is the corresponding author.
% We thank all  SAFARI Research Group members, especially Skanda Koppula, for  insightful feedback. 

% , the National Natural Science Foundation of China (NSFC) under Grant No. 62032020, and the Tsinghua University Initiative Scientific Research Program.
% This work is also supported in part by the NSFC under Grant No. 2023YFB4502902.


==> texfile/11_ae.tex <==
% LaTeX template for Artifact Evaluation V20240722
%
% Prepared by Grigori Fursin with contributions from Bruce Childers,
%   Michael Heroux, Michela Taufer and other colleagues.
%
% See examples of this Artifact Appendix in
%  * ASPLOS'24 "PyTorch 2: Faster Machine Learning Through Dynamic Python Bytecode Transformation and Graph Compilation": 
%      https://dl.acm.org/doi/10.1145/3620665.3640366
%  * SC'17 paper: https://dl.acm.org/citation.cfm?id=3126948
%  * CGO'17 paper: https://www.cl.cam.ac.uk/~sa614/papers/Software-Prefetching-CGO2017.pdf
%  * ACM ReQuEST-ASPLOS'18 paper: https://dl.acm.org/citation.cfm?doid=3229762.3229763
%
% (C)opyright 2014-2024 cTuning.org
%
% CC BY 4.0 license
%


\appendix
\section{Artifact Appendix}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Abstract}
We implement Gaze using ChampSim simulator~\cite{ChampSim}.
In this artifact, we provide all the necessary information to reproduce the main experiments presented in the paper. We describe how to prepare the required datasets, set up the system, and run the artifact. This artifact includes the source code of the ChampSim simulator used in our experiments and the scripts to build all binaries, run the experiments, and draw figures. 

\subsection{Artifact check-list and meta-information}

{\small
\begin{itemize}
  \item {\bf Program:} ChampSim
  \item {\bf Compilation:} G++ 11.4.0
  \item {\bf Data set:} Traces from SPEC06~\cite{SPEC06}, SPEC17~\cite{SPEC17}, Ligra~\cite{Ligra}, PARSEC~\cite{PARSEC}, CloudSuite~\cite{CloudSuite}, QMM~\cite{CVP1}, and GAP~\cite{GAP} benchmark suites.
  \item {\bf Hardware:} No specific hardware requirements.
  \item {\bf Output:} 15 PDF figures.
  \item {\bf How much disk space required?} $\sim$100GB
  \item {\bf How much time is needed to prepare workflow?} $\sim$2 hours, including downloading traces.
  \item {\bf How much time is needed to complete experiments?} $\sim$7-10 days when using a compute cluster with 384 cores: key single-core results (1 day, fig. 1, 6-8, 11), multi-core results (4-5 days, fig. 14-15), supplementary single-core results (2-3 days, fig. 4, 9, 10, 12-13, 16-18).
  \item {\bf Publicly available?} Yes
  \item {\bf Code licenses (if publicly available)?} GPL-3.0
  \item {\bf Archived (provide DOI)?} \href{https://doi.org/10.5281/zenodo.14252372}{10.5281/zenodo.14252220}
\end{itemize}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Description}

\subsubsection{How to access}
The source code can be obtained from GitHub: \href{https://github.com/SJTU-Storage-Lab/Gaze-Spatial-Prefetcher.git}{https://github.com/SJTU-Storage-Lab/Gaze-Spatial-Prefetcher.git}

\subsubsection{Hardware dependencies} 
No specific hardware requirements. Gaze can be run on any system with a general-purpose CPU.

\subsubsection{Software dependencies}
Gaze is tested on Ubuntu 18.04. The following dependencies are recommended:

\begin{itemize}
    \item Ubuntu 18.04.6 LTS
    \item Linux Kernel 5.4.0-150-generic
    \item G++ 11.4.0
    \item Python 3.8.18
    \begin{itemize}
        \item matplotlib 3.7.2
        \item numpy 1.24.3
        \item pandas 2.0.3
        \item scipy 1.10.1
    \end{itemize}
\end{itemize}

\subsubsection{Data sets}
The traces used in our experiments are primarily from championships or previous work. Below is the detailed information about obtaining these traces. They should be manually downloaded. 

\begin{itemize}
    \item \textbf{SPEC06 and SPEC17 traces.} Available from DPC-3~\cite{DPC3} (\url{https://dpc3.compas.cs.stonybrook.edu/}).
    \item \textbf{PARSEC and Ligra traces.} Originally from Pythia~\cite{Pythia} (not available now), we have archived a copy of our used traces.
    \item \textbf{CloudSuite traces.} Available from CRC-2~\cite{CRC2} (\url{https://crc2.ece.tamu.edu/}).
    \item \textbf{GAP traces} (only used in supplementary experiments). Archived.
    \item \textbf{QMM traces} (only used in supplementary experiments). Archived.
\end{itemize}

All traces should be placed directly in the trace directory \texttt{\$GAZE\_HOME/traces}.

Run the following command to check if the required traces are ready.
\begin{verbatim}  
    $ cd $GAZE_HOME/scripts   
    $ python trace_check.py
\end{verbatim} 

\subsection{Installation}

\vspace{5pt}
1. Clone Gaze from GitHub repository
\begin{verbatim}  
    $ git clone   
\end{verbatim} 


Gaze is implemented in ChampSim, thus, ChampSim needs to be successfully built. The following are the build steps from \texttt{ChampSim/README.md}. For more detailed information, please refer to it.

\vspace{5pt}
2. Download ChampSim's dependencies
\begin{verbatim}  
    $ cd ChampSim
    $ git submodule update --init
    $ vcpkg/bootstrap-vcpkg.sh
    $ vcpkg/vcpkg install  
\end{verbatim} 

Then, we can compile all prefetchers.

\vspace{5pt}
3. Build all binaries
\begin{verbatim}  
    $ cd ../scripts/make
    $ python make_all.py
\end{verbatim} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Experiment workflow}
This section lists instructions to execute experiments. 
The running and plotting scripts are located in \texttt{scripts/run} and \texttt{scripts/draw}, respectively.
The simulation will generate raw log and json files that will be used for figure plotting.
Some eight-core heterogeneous simulations take more than four days to complete, therefore, please allocate dedicated CPU resources for multi-core heterogeneous simulations.
% A single running script launches multiple experiments simultaneously. It can be modified to start only a subset of experiments. 
Each script launches all corresponding simulations at once, which may occupy excessive system resources. It can be modified to run only a subset of the simulations.
After manually confirming that the relevant simulations have completed, the plotting script can be executed to generate the figure. 

\vspace{5pt}
1. Main single-core simulations (fig. 1, 6-8, 11)
\begin{verbatim}  
    $ cd $GAZE_HOME/scripts/run
    $ python run_single_core_main.py
    $ # wait for simulation
    $ cd ../draw
    $ python fig1.py # fig/fig1.pdf
\end{verbatim} 

\vspace{5pt}
2. Multi-core homogeneous simulations (fig. 14a)
\begin{verbatim}  
    $ python run_multi_core_homo.py
\end{verbatim} 

\vspace{5pt}
3. Multi-core heterogeneous simulations (fig. 14b, 15)
\begin{verbatim}  
    $ python run_multi_core_hete.py
\end{verbatim} 

4. Supplementary simulations (fig. 4, 9, 10, 12-13, 16-18)
\begin{verbatim}  
    $ python the_running_script.py 
\end{verbatim} 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Evaluation and expected results}

The simulation does not directly output results. Instead, it writes the raw data to a json file, which is saved in \texttt{GAZE\_HOME/json} directory. Meanwhile, runtime logs are stored in \texttt{GAZE\_HOME/log}.
The plotting scripts convert the raw data into result data and generate the figures included in the paper.
Therefore, the generated figures should be consistent with those presented in the paper.

\subsection{Notes}
Before generating a figure, please ensure all corresponding simulations have completed. This can be manually verified through process status or the associated logs (in \texttt{log}).
This is because, in a few multi-core simulations, ChampSim actively terminate due to invalid simulation states, which can result in invalid raw data. Thus, the plotting code is designed to handle invalid log and json files. However, not all invalid files are generated from active termination; some are invalid because the simulations remain unfinished.


==> texfile/3_back_and_moti-HP.tex <==
\section{Related Works and Motivation}
\label{sec:background}


% Hardware prefetchers leverage the observed access pattern to predict the subsequent memory access and fetch the blocks prior to explicit CPU demands, thus eliminating the long data access latency.

% In this section, we first briefly introduce the basics of some state-of-the-art prefetchers. Next, we describe how bit-pattern-based prefetcher.
% In this section, we give a brief overview of region-based prefetching. We then use this as an example to illustrate how the aggressiveness and the resulting speedup have been increasing. 
% Finally, we briefly introduce the features and advantages of bit-pattern-based prefetching.

% In this section, we give a brief overview of recent spatial prefetching. 
% We then discuss why its underlying pattern index scheme is a weak link.


%{\footnote{{When representing the construction of events, we interchangeably use terms `construct', `extract' and `form', all of which convey the same meaning.}}}
% \subsection{Spatial-Pattern-based Prefetching} \label{subsec:bit-pattern-based_prefetching}
%     Spatial-pattern-based prefetching learns the spatial pattern of a certain region (e.g., a physical page) through directly recording its footprint~\cite{SPP_04,SFP}. It keeps track of all recently activated regions. For each $n$-block region, an $n$-bit vector is used to indicate whether each data block has been accessed, which we call \textit{spatial pattern}. For example, suppose there is an eight-block region $A$. After accessing the blocks $A+2$, $A+3$ and $A+6$, a bit vector $00110010$ will be seen. After the region becomes inactive, its spatial pattern is generated and is associated with an event which activated its generation. This event is typically constructed by combining various features from the trigger demand access, including the Program Counter (PC) of this trigger memory instruction, the memory address, and the offset from the start of the region\footnote{In line with previous studies~\cite{SPP_04,SMS,Bingo,PMP,DSPatch}, for brevity, we refer to it as \textit{offset} in the rest of this paper.}. 


%     When an active region is likely to exhibit a similar spatial pattern to a previously accessed region, the prefetching is then called. Specifically, whenever activating an inactive region, the event extracted from this trigger access is used to search the past patterns. Once a match is found, the pattern is used to predict the possible future accesses. For example, when using \texttt{`PC+Address'}, the recurrence of a certain event means that the same instruction is used to touch the same address, which indicates that the stored corresponding pattern is pretty likely to replay.


% To perform prefetching, whenever accessing a new spatial region, the event extracted from this trigger access is used to search the past patterns. Once a match is found, which means that this region is likely to exhibit a similar spatial pattern, the pattern is used to do prefetching.

% Whenever accessing a new spatial region, the event extracted from this trigger access is constructed and then used to search the past patterns. Once a match is found, which means that this region is likely to exhibit a similar spatial pattern, the pattern is used to do prefetching.

% Once a bit pattern is generated, i.e., the tracking of the region ends, the bit-pattern-based prefetcher associates it with an event which is extracted from the trigger access (i.e., the first access to the region). And whenever the event reoccurs, the pattern is used to perform prefetching.

% As shown in Fig.~\ref{fig:SMS}, recent spatial prefetchers commonly consist of three main components: Filter Table (FT), Accumulation Table (AT), and Pattern History Table (PHT)~\cite{SMS,Bingo,PMP}. FT is used to filter out the one-bit spatial pattern, which indicates that only one block in the region is fetched during the recording. AT is used to track all active regions, and PHT is used to store event-pattern pair, which is generated after the accumulation. Any newly activated region is first recorded in the FT and will be tracked only after the arrival of the second different access. Moreover, recent spatial prefetchers typically employ a Prefetch Buffer (PB) to efficiently store the prefetch addresses, as a single bit vector often contains multiple requests with the same starting address. In addition, PB also helps to smooth the issuance of prefetches. 

% A significant minority of spatial region generations never have a second block accessed; there is no benefit to predicting these generations because the only access is the trigger access.

% \begin{figure}[htb]
%     \centering
%     \includegraphics{figure/SMS.pdf} % [width=0.45\textwidth]
%     \caption{Structure of region-based prefetching. {\em H}/{\em M} represents a hit/miss in the corresponding table.} 
%     \label{fig:SMS}
% \end{figure}

% Upon arrival of an access, the prefetcher initially checks AT to see if the accessed region is under tracking (\ding{202}), and if so, the prefetcher updates the corresponding footprint; otherwise, the prefetcher looks up the FT (\ding{203}), and if the region is found, which means that it has been activated once before, the prefetcher then starts tracking it in AT (\ding{204}); and if it is not found, which indicates that the region is now activated and this access is also a trigger access, the prefetcher records it in FT and then uses the event constructed based on this access to search the PHT to determine whether to do prefetching (\ding{205}). If there is a match in PHT, the corresponding spatial pattern is sent to PB, ready for prefetching (\ding{206}). For each region that is under tracking, once it becomes inactive (i.e., one of its words  is evicted/invalidated, or there is no demand to this region for a long time), the accumulation ends and the bit vector is sent to PHT (\ding{207}).


\subsection{Recent Spatial-Pattern-based Mechanisms}
\label{subsec:recent_prefetching_mechanisms}
Spatial-pattern-based prefetching learns the spatial pattern of a certain region through directly recording its footprint and tries to find other similar regions to deploy the learned experience for prefetching~\cite{SPP_04,SFP}. The potential of it has been demonstrated by many prior works~\cite{SFP,StealthPrefetching,SPP_04,DSPatch,SMS,SMS_R,Bingo,PMP,BuMP,STeMS}.
% First, a bit vector provides a global view for all accesses to the region, thereby eliminating the impact of out-of-order scheduling~\cite{DSPatch}. Second, spatial prefetching is particularly beneficial in scenarios where there are similar loops, structures with repetitive data layouts, and data structure traversals~\cite{Primer,SMS,SMS_R,PMP,Bingo}. In addition, spatial prefetchers directly replays the past accesses of the region, making it more adaptable, especially for some patterns that are intuitively difficult to identify. 


Spatial Footprint Predictor (SFP)~\cite{SFP} first exemplifies the common structure and logic of spatial-pattern-based prefetching. SFP proposes to use PC as well as some bits from the data address to characterize patterns, which improves the prefetch accuracy and enables the prefetcher to eliminate compulsory misses. Spatial Pattern Prediction~\cite{SPP_04} improves SFP with larger region size and cache line size.

\textbf{Fine-grained spatial prefetching} typically characterize patterns with several environmental contexts such as the activating instruction \textit{and} data address.
Spatial Memory Streaming (SMS)~\cite{SMS} proposes to use \texttt{`PC+Offset\footnote{Offset means the distance of the block address from the beginning of a region.}'}. SMS also uses a filter table (FT) to filter out one-bit spatial footprints. Bulk Memory Access Prediction and Streaming~\cite{BuMP} further reduces the energy consumption of SMS.
% 细粒度的预取通常同时使用触发访问的指令和地址来形成事件。

Bingo~\cite{Bingo} is motivated by the fact that the shorter contexts (\texttt{`PC+Offset'}) is carried in the longer one (\texttt{`PC+Address'}). Inspired by the TAGE~\cite{TAGE} branch predictor, Bingo first tries to use the longer trigger contexts to find the exact match. If it is not found, then the shorter contexts is used to find the approximate match.
Therefore, compared to SMS, Bingo achieves similar accuracy (sustained by exact matches) with more misses being covered (approximate matches).
% , i.e., those with the same shorter event are used together for prefetching.
% To reduce redundancy, Bingo uses \texttt{`PC+Offset'} as the index and uses \texttt{`PC+Address'} as the tag to index patterns. 
% An approximate match means that all the patterns with the same shorter event are used together for prefetching.
% , which increases the aggressiveness. 

Using various environmental contexts accurately characterizes the system-level features where the pattern begins. Therefore, the prediction for a matched region typically has a high accuracy.
However, similar patterns often occupy distinct storage spaces due to minor contextual differences, causing severe data redundancy~\cite{Bingo, PMP}.
Thus, it requires extremely high storage overhead and lengthy learning period to achieve high coverage~\cite{PMP,DSPatch}, which makes the prefetcher impractical. Both SMS and Bingo require more than 100KB of storage when they achieve their optimal performance~\cite{SMS,Bingo}.

\textbf{Coarse-grained spatial prefetching.} To this point, several recent studies attempt to do it in simpler ways. They opt for coarse-grained events that are more hardware-friendly, and employ various methods to mitigate the resulting low accuracy.
Coarse-grained methods characterize patterns with only a few bits from the trigger instruction \textit{or} data address.

% 粗粒度的预取通常只使用触发访问的指令或地址的少量位来形成事件。

Dual Spatial Pattern Prefetcher (DSPatch)~\cite{DSPatch} characterizes spatial patterns at the granularity of instructions (i.e., \texttt{`PC'} is used). At the same time, it maintains two up-to-date patterns for each PC and can further improve accuracy/coverage by prefetching data blocks that appear in both/either pattern.

Pattern Merging Prefetcher (PMP)~\cite{PMP} further coarsens the characterization by using only the \texttt{`Offset'}, ensuring that a match can almost always be found after working for a short period. This almost minimizes the chances of losing prefetch opportunities due to the execution of new instructions or access to unseen addresses.
In addition, for each offset, PMP merges the 32 most recent patterns, meaning that their common features are preserved and utilized.
% However, this also implies that patterns, which are no longer used, can still trigger prefetching for an extended period. 
% leading to a significant number of useless prefetches. 

\subsection{Existing Limitations and Motivation}
% As shown in Fig.~\ref{fig:single_multi}, only fine-grained SMS and Bingo successfully achieve balanced performance. However, both they incur huge on-chip area and long access time~\cite{PMP}. On the other hand, coarse-grained characterization, which is more hardware-friendly, makes different spatial patterns are more likely to have the same event. When such a conflict occurs between the old and the new, the prefetcher lacks the ability to judge which pattern is better.

Conventional context-based methods exhibit significant limitations in capturing key access characteristics. As shown in Fig.~\ref{fig:single_multi}, low-cost solutions are challenging to apply to complex workloads, while introducing more environmental contexts can lead to prohibitive hardware costs. Although numerous efforts have been made to mitigate this inefficiency, their shortcomings remain unresolved. It would be desirable to take a deep look into the patterns themselves so that we can better understand how to characterize them efficiently.

% We observe that the access order exhibited within the footprint plays a crucial role in characterizing spatial patterns.

% Since access behavior often exhibit temporal correlations within themselves~\cite{temporal_correlation}. we examine the spatial patterns generated by them should also share similar properties.
Memory access often exhibits temporal locality, meaning that accessed data are likely to be reused in the near future~\cite{Primer}.
Temporal correlation, as an analog to temporal locality, refers to the phenomenon where a group of addresses tends to be reused \textit{in the same order}~\cite{temporal_correlation}. It is widely used in identifying irregular patterns such as pointer chasing, graph processing, and so on~\cite{STeMS,Markov,STMS,GHB,ISB,Domino,Triage,MISB}.
% Cache hierarchy and temporal prefetchers rely deeply on this property.
Since spatial patterns are generated by memory access, they should also exhibit similar temporal properties within themselves.
Inspired by this fact, we find that when spatial pattern recurs, data blocks are likely to be accessed in a similar order.


\begin{figure}[h]
    \vspace{-2pt}
    \centering
    \includegraphics{figure/order.pdf} % [width=0.45\textwidth]
    \caption{The detailed reference footprints of several spatial regions. These regions are accessed close in time. The trigger accesses are cycled in red. The footprint of region \textit{B} is partially given.
    }
    \label{fig:order}
    \vspace{-10pt}
\end{figure}


The upper part of Fig.~\ref{fig:order} provides an example obtained from \texttt{fotonik3d\_s}. It plots detailed footprints of three spatial regions. The spatial footprints as well as their internal temporal correlations exhibited in region \textit{A} and region \textit{C} are the same. That is, their referenced blocks are aligned and are accessed in the same order.
In contrast, region \textit{A} and region \textit{B} show significant differences in terms of both spatial footprints and access orders.

% Compared to trigger contexts, this type of internal features is more intrinsic in characterizing spatial patterns. 
% 相比于程序上下文这种外部特征，空间足迹内部的时间局部性是由访问行为本身产生的。因此，它能够更本质地刻画出访问特征。
Since footprint-internal temporal correlations are access-intrinsic, utilizing them for fine-grained characterization could be a feasible direction. As shown in Fig.~\ref{fig:order}, suppose region \textit{A}, \textit{B} and \textit{C} have been deactivated recently (their patterns have been learned) and region \textit{D} is just activated at time $t_0$. The trigger accesses of these four regions, which are cycled in red, are aligned. Thus, they are similar by definition. However, the patterns of region \textit{A}, \textit{B} and \textit{C} have met a conflict. At this time, the prefetcher should choose a pattern for prefetching in region \textit{D}. But how would we decide which pattern to use? Introducing additional contexts like PC could help, but the cost would be unacceptable. We answer this by the help of the footprint-internal temporal correlation. Before making decision, we need to wait for more subsequent accesses to extract their temporal correlation. As shown in Fig.~\ref{fig:order}, after waiting for two subsequent accesses to this region (time $t_2$), we can clearly see that the similarity between region \textit{B} and region \textit{D} is very high. Thus, at time $t_2$, we can make a high-confidential prediction.

However, this idea is not readily applicable to spatial-pattern-based prefetching. This is primarily due to \ding{202} its incompatibility with conventional hardware designs and \ding{203} the additional complexity it introduces.
The first challenge arises because conventional methods make predictions based on trigger accesses, but multiple observations are required to obtain temporal correlations. Moreover, footprints are stored as bit vectors, which retains only spatial information while completely discarding temporal features. The second challenge is that storing and utilizing temporal information inevitably introduces extra complexity. If not utilized properly, the effectiveness may be inferior to previous fine-grained approaches.
Therefore, to maintain simplicity and efficiency, we need a careful design.
% This also means a loss of prefetching opportunities, as we need to wait for multiple accesses before making predictions. 



% extracting internal features from newly-activated regions is challenging, as only a tiny portion of their footprints can be observed when predicting. Besides, there are several sources of inefficiency.
% For instance, the incompatibility with conventional hardware designs, as % 它们从没尝试过使用内部特征
% footprints are stored as bit vectors, which retains only spatial information while completely discarding temporal features.
% Therefore, to maintain simplicity and efficiency, we need a careful design.

% thanks to the use of fine-grained event for accurately identifying similar regions,
% 如图1所示，Bingo实现了完美的性能平衡。
% 但是，其16k-entry的模式表需要巨大的面积和过长的访问时间，这限制了它的实际使用。
% 对快速且珍贵（单位面积非常昂贵）的片上缓存，尤其是L1D，而言，一个小且简单的模式表才是合适的。

% 粗粒度地索引模式对硬件更加友好，但也意味着不同的模式很容易冲突。当新旧模式发生冲突时，预取器没有更多的信息来判断哪个更有可能在将来被使用，因此它们通常合并发生冲突的模式。然而，拥有相同较短触发事件的区域仅拥有适量的相似性，这对高性能预取而言是远远不够的。DSPatch根据带宽占用动态地利用两个冲突的历史模式。PMP使用复杂的机制，对长达32个冲突的历史模式提取共同特征。但是如图所示，它们收效甚微。显然，合并冲突的模式并不是一个理想的解决方案，它并没有从根本上将冲突区分开。

% 模式发生冲突是因为短的触发事件不足以 characterizing the access patterns.

% Relying solely on PC cannot capture multiple patterns that are generated by the same instruction. Using the higher bits of data address (e.g., the region number) makes it difficult to identify other similar pages while focusing on the lower bits (e.g., the offset) can lead to numerous mispredictions.

% Spatial-pattern-based prefetching predicts the upcoming footprint by identifying past regions that are similar to the candidate region.
% However, conventional environmental-context-based identifying is not particularly effective. For instance, relying solely on the program counter (PC) can lead to inefficiencies when a single instruction results in multiple spatial patterns. Using only the higher bits of an address, which represent the region number, makes it challenging to identify other similar pages; conversely, focusing solely on the lower bits (i.e., offsets) can lead to the misapplication of spatial patterns in inappropriate areas. While combining both instruction and address is a viable approach, it incurs significant hardware overhead. Although recent methods have introduced various optimization strategies, these still fundamentally rely on traditional feature extraction, resulting in improvements that remain inefficient rather than fully addressing the issue.

% Moreover, it is important to note that internal characteristics of the patterns themselves can also be leveraged. To date, however, research focusing on using internal features from the footprint for prediction has been limited. Extracting internal features from a complete footprint is relatively straightforward, but applying these features to newly activated regions poses a challenge, as the footprints for these regions often reveal only a fraction of the information. This indicates that exploring and utilizing these internal characteristics could present a new design opportunity aimed at enhancing the accuracy and efficiency of spatial prefetching.


% % The key to spatial footprint prediction lies in the ability to accurately characterize access patterns. 
% Conventional context-based methods exhibit significant limitations in capturing the key characteristics of access behavior. Relying solely on PC cannot capture multiple patterns that are generated by the same instruction. Using the higher bits of data address (e.g., the region number) makes it difficult to identify other similar pages while focusing on the lower bits (e.g., the offset) can lead to numerous mispredictions.


% Current spatial-pattern-based prefetchers predominantly rely on conventional environmental contexts, such as the program counter (PC) and data address. While these features are instrumental in characterizing memory access patterns, they are insufficient in capturing the full complexity of access behavior. A significant limitation arises from the inherent characteristics of instructions that can generate multiple spatial patterns. For instance, a single instruction may access various memory regions, rendering reliance on just the PC ineffective. Similarly, using only the high bits of the address (i.e., the region number) complicates the identification of other similar patterns due to the limited information provided. On the other hand, focusing solely on the lower bits (the offset) often leads to prefetched data residing in incorrect address spaces, diminishing the overall accuracy and efficiency of the prefetching process. Although combining both instruction and address offers a potentially more robust solution, it introduces substantial overhead that can negate the performance benefits.

% Moreover, while recent advancements have proposed various optimizations, these methods still fundamentally rely on traditional characteristic features, thus only marginally improving efficiency without addressing the root causes of the limitations. One unexplored avenue is the potential of incorporating internal features of the memory access pattern itself. The internal characteristics of memory access patterns could provide valuable insights that are not captured by environmental contexts alone. Although past methodologies have primarily focused on external features, leveraging these internal attributes could significantly enhance prediction accuracy.

% It is important to note that extracting internal features from complete spatial footprints is feasible; however, applying these features to newly activated regions poses a considerable challenge due to the limited visibility of previous memory accesses.

% In summary, there remains a critical need to move beyond conventional environmental context-based features to embrace a dual approach that incorporates both environmental and internal characteristics. This shift could enable more effective footprint prediction, especially in complex workloads characterized by diverse access patterns. By investigating and integrating these internal features, new prefetching designs could mitigate existing inefficiencies and unlock improved performance in memory access predictions, paving the way for more sophisticated and effective hardware prefetching strategies.


% As shown in Fig.~\ref{fig:single_multi}, only Bingo successfully achieves the {balanced} performance. However, its 16k-entry pattern history table (PHT) requires huge on-chip area and long access time~\cite{PMP}. For fast and precious on-chip caches, especially the L1D, we need a small and simple PHT.

% Coarse-grained characterization is more hardware-friendly. But it brings a new challenge: different spatial patterns are more likely to have the same event. When such a conflict occurs between the old and the new, the prefetcher lacks the ability to judge which one is better. One commonly used low-cost method is merging~\cite{DSPatch, PMP}. However, the moderate similarity among conflicted regions is insufficient for high-performance prefetching.

% DSPatch dynamically merges the last two conflicted patterns. PMP employs a more complex mechanism. It extracts common features from up to 32 conflicted patterns. However, as shown in Fig.~\ref{fig:single_multi}, their effectiveness is minimal. Thus, merging conflicted patterns is not an ideal solution as it does not fundamentally tell conflicts apart.

% Although several recent low-cost prefetchers fail to achieve outstanding performance, they have shown tremendous potential to us. We try to distill the underlying limitation from them and then see a new possibility for achieving a beautiful low-cost solution.

% \textbf{The underlying limitation.} We argue that the fundamental weak link is their pattern index scheme. All these proposals
% % utilize environmental features from where the pattern generation begins to index its possible spatial pattern. In other words, they 
% use the event extracted from the trigger access to index patterns. But it is inefficient in characterizing access patterns. In order to make accurate predictions while covering adequate demand requests, the prefetcher would need unaffordable hardware cost. Low-cost solutions, on the other hand, are difficult to scale to various scenarios due to the negative gains stemmed from their low accuracy and high aggressiveness.

% \textbf{The underlying limitation.}
% {Previous methods attempt to find a reasonable granularity to utilize trigger contexts. However, as illustrated in Fig.~\ref{fig:single_multi}, their performance falls short of expectations. Low-cost solutions are difficult to scale to various scenarios while introducing more environmental contexts could incur prohibitive hardware expenses. Therefore, we conclude that their underlying pattern characterization scheme---\textit{relying exclusively on environmental trigger features}---is cost-ineffective. In this paper, we aim to identify a more intrinsic feature to effectively characterize access behaviors.}

==> texfile/4_moti.tex <==
\section{Gaze Spatial Prefetcher}
\label{sec:gaze_spatial_prefetcher}

We propose Gaze, which to our best knowledge is the first spatial prefetcher that utilizes \textbf{footprint-internal temporal correlations} to efficiently characterize spatial patterns.
To balance hardware complexity and performance, Gaze leverages information from region's first two accesses (\S\ref{subsec:Pattern Characterization}). This simplification allows Gaze to seamlessly integrate temporal feature extraction into existing hardware designs without extra metadata storage.
At the same time, Gaze introduces a dedicated two-stage approach to mitigate the over-prefetching problem that often occurs in conventional schemes when they utilize high-dense footprints generated from spatial streaming (\S\ref{subsec:Enhancement towards Spatial Streaming}).

{Gaze is designed and primarily evaluated as an L1D prefetcher. Nevertheless, it can also be placed at L2C,} working in conjunction with the existing commercial L1D prefetcher {IP-stride}.

% Gaze is designed as an L1D prefetcher. Since spatial footprint prediction is robust against the incompleteness of access sequence, Gaze can also be placed at L2C, working in conjunction with the existing commercial L1D prefetchers.

% 0 0 0 0 0 0 1 2 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 3 4 5 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0

% 4 5 0 0 0 0 1 6 7 8 9 10 11 12 13 14 15 16 17 18 19 20 21 22 23 24 25 26 27 28 29 30 31 0 0 3 2 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0 0



\subsection{Design Overview}

\begin{figure*}[htb]
    % \vspace{-3pt}
    \centering
    \includegraphics{figure/Gaze_new.pdf} % [width=0.45\textwidth]
    \caption{Design overview of Gaze (b) and its detailed learning (a) and prefetching (c) process. For simplicity, we use \textit{trigger} and \textit{second} to refer to the trigger offset and the second offset, omitting the term \textit{offset}. \textit{H} and \textit{M} mean a hit and a miss in the corresponding structure, respectively.}
    \label{fig:Gaze}
    \vspace{-10pt}
\end{figure*}

% 图3b是Gaze的设计概览。

% TODO 0801
Fig.~\ref{fig:Gaze} illustrates the design of Gaze. The middle sub-figure (Fig.~\ref{fig:Gaze}b) shows the design overview, while the left sub-figure (Fig.~\ref{fig:Gaze}a) and the right sub-figure (Fig.~\ref{fig:Gaze}c) illustrate the detailed learning and prefetching procedure, respectively.
The key innovations, including the use of the temporal information from the first two accesses (the detail is discussed in \S\ref{subsec:Pattern Characterization}) and the path of dedicated aggressiveness control (\S\ref{subsec:Enhancement towards Spatial Streaming}), are highlighted in Fig.~\ref{fig:Gaze}b.

As shown in Fig.~\ref{fig:Gaze}b, Gaze is trained on cache loads.
Similar to conventional spatial-pattern-based prefetchers{~\cite{Bingo, PMP, SMS}}, Gaze consists of three main components: Filter Table (FT), Accumulation Table (AT), and Pattern History Module (PHM). FT is used to filter out one-bit spatial patterns, indicating that only one block in the region is demanded during tracking. AT is used to track all active regions. PHM is used to learn access pattern, and to issue prefetches based on the learned experience. Any newly activated region is first recorded in FT and will be tracked by AT only after the arrival of the second different load access. Gaze also employs a Prefetch Buffer (PB) to efficiently store the prefetch addresses, as a single bit vector often contains multiple requests with the same starting address, i.e., the region number. In addition, PB also helps to smooth the issuance of prefetches.

\textbf{Access Flow.} Upon the arrival of a {load}, Gaze initially checks AT to see if the accessed region is under tracking (\ding{202}), and if so, Gaze updates the corresponding footprint.
Otherwise, Gaze looks up the FT (\ding{203}). If the region is found, which means that it has been activated once before, Gaze then starts tracking it in AT (\ding{204}).
Unlike previous proposals, Gaze will also send the trigger offset, the second offset as well as the trigger PC to PHM for prefetching (\ding{205}). This is because Gaze chooses to incorporate the temporal correlation between the first two accesses, which is available at this point. If more accesses are required, this step would be delayed.
Conventional methods{~\cite{Bingo, PMP, SMS, DSPatch}} awaken the prefetching process through the trigger access rather than the second access.
After receiving these, PHM decides whether to trigger prefetching for this region. If so, the corresponding prefetch pattern will be sent to PB, ready for prefetching (\ding{206}).  For each region that is under tracking, once it is deactivated (e.g., one of its cached blocks is evicted out of the cache, 
or its associated tracking entry is evicted from the AT by the LRU policy due to inactivity), the accumulation ends and the bit vector is sent to PHM (\ding{207}) for pattern learning.


Each entry in the AT is used to track an active region, where we introduce two additional 6-bit fields to store the offsets of the region's last two accesses, which, together with the new access, will collectively calculate the last two strides. AT decides whether to perform region-based stride prefetching (used as the backup prefetching) and aggressiveness promotion based on the two strides (\ding{208}).
% This will be discussed in \S\ref{subsec:Two-Stage Aggressiveness Promotion}.


\subsection{Pattern Characterization}
\label{subsec:Pattern Characterization}


To identify footprint-internal features, Gaze has to wait for several initial accesses.
%  to extract their temporal correlation.
% Then, Gaze selects the most similar pattern from multiple distinct candidates under the same trigger short event.
Thus, the most critical design choice is the number of accesses used for temporal correlation extraction. 
This requires Gaze to hold and observe all recently activated regions, differentiating their spatial patterns based on their recently accessed blocks in the presence of strong interference such as out-of-order scheduling. Besides, this also means the loss of prefetch opportunities. Therefore, waiting for too many accesses incurs negative effect.

% For hardware simplicity, Gaze is based on coarse-grained event, namely, the \texttt{`Offset'}, which incurs low hardware cost.
% Specifically, Gaze maintains multiple distinct candidates under the same trigger offset. When an inactive region is activated, Gaze does not issue prefetches immediately. Instead, Gaze wait for several subsequent accesses to make exact prediction based on their temporal correlation. From an implementation perspective, Gaze uses the trigger offset as the index and in-pattern temporal information as the tag.

% 
% Fortunately, we find that utilizing the temporal correlation among a few initial accesses can achieve a decent pattern characterization. Furthermore, it can naturally integrate with previous pattern index scheme. These enable Gaze to maintain hardware simplicity while attaining high accuracy 

% To keep the hardware simplicity, Gaze is based on coarse-grained event \texttt{`Offset'}. 


% Fortunately, we find that utilizing the temporal correlation among a few initial accesses can achieve a desired level of pattern differentiation. Fig.~\ref{fig:sms_varying_offsets} shows the accuracy, coverage, and speedup achieved by several spatial-temporal co-. They discard the PC when forming the event and extend the number of accesses required before prefetching from one to up to four. Meanwhile, to keep things simple, they directly use these offsets to index patterns. When only the trigger offset is used, the size of the PHT is 64 since {we only have 64 distinct offsets within a 4KB region}. But when using two or more accesses, a full PHT is impractical and inefficient. Therefore, we use 256-entry fully-associative history tables in these cases for simplicity, which consumes less than 3KB.\footnote{The performance is saturated after the size is larger than 256.}

% Notably, our findings indicate that leveraging the temporal correlation among a limited number of initial accesses can achieve a desired level of pattern characterization. 
% 为了确定所需要的初始访问次数，我们首先研究性能与之的关系，以获取一个优秀的平衡。
% in terms of speedup, prefetch accuracy and miss coverage. and the number of accesses to find a desirable balance.
To strike a good performance-cost balance, we first explore the relationship between the amount of temporal information used and the resulting efficiency in terms of speedup, accuracy, and coverage. 
We say two regions are similar when their initial accesses are aligned in both spatial footprint and temporal order. Fig.~\ref{fig:sms_varying_offsets} illustrates the effect of extending the number of aligned initial accesses required from one to up to four. The results are the averages across the entire evaluation set. We sequentially concatenate the offsets of these accesses to form the index event. When only the trigger offset is used, the size of the pattern history table (PHT) is 64, since there are 64 distinct offsets within a 4KB region {and no instruction information is incorporated}. However, when considering more accesses, a full PHT becomes impractical and inefficient. Therefore, for simplicity, we use 256-entry fully-associative history tables in these cases, which consume less than 3KB.\footnote{The performance is saturated after the size is larger than 256.}

\begin{figure}[htb]
    % \vspace{-11pt}
    \centering
    \includegraphics{figure/sms_varying_offsets.pdf} % [width=0.45\textwidth]
    \caption{Effect of extending the number of aligned initial accesses that required for a match. The region size is set to 4KB.}
    \label{fig:sms_varying_offsets}
    % \vspace{-10pt}
\end{figure}

As illustrated in Fig.~\ref{fig:sms_varying_offsets}, if we require that the first four demanded blocks must be aligned both spatially and temporally, the prefetch accuracy increases from 56\% to 90\%, indicating the successful characterization of access behaviors.
However, prefetch opportunities are substantially lost, resulting in a decrease in IPC and coverage. An ideal balance is achieved when we choose to only use the first two accesses, which provides a 3\% improvement in IPC and a 35\% improvement in accuracy, with only negligible reduction in coverage. When the number of used offsets increases again, a marginal gain in accuracy comes at a cost of a significant degradation in both IPC and coverage.

Building on this insight, we decide to leverage the temporal correlation between the first two accesses to characterize spatial patterns. This choice offers three major advantages.
{Firstly, this approach significantly reduces storage overhead compared to conventional fine-grained methods that rely on diverse program contexts.}
Secondly, it balances performance, accuracy, and coverage, ensuring timely prefetches and minimizing interference from out-of-order scheduling. 
Thirdly, it can be seamlessly integrated into recent hardware designs.
Gaze utilizes existing logic to capture the first two offsets and store patterns in a way that does not cost extra metadata overhead, maintaining simplicity and compatibility.
Specifically, recent methods employ FT to invalidate the regions that are accessed only once, which allows us to obtain these two offsets when FT sends a valid region to AT (\ding{205} in Fig.~\ref{fig:Gaze}b). Additionally, we use the first offset as the index and the second offset as the tag to store patterns, with their order inherently verified during the table lookup process.

% This synergy enables highly efficient prefetching, with significant accuracy gains and negligible coverage reduction.

% The first advantage is that it strikes a favorable balance among performance, accuracy and coverage, while also ensuring that prefetches are not significantly delayed. Meanwhile, it effectively mitigates the interference from out-of-order scheduling.

% Another advantage is that it can be seamlessly integrated into recent hardware designs. This is achieved through two adaptations. Firstly, the first two offsets can be readily captured using existing logic. Recent methods employ FT to invalidate the regions that are accessed only once. This allows us to obtain these two offsets when FT sends a valid region to AT (\ding{205} in Fig.~\ref{fig:Gaze}b).
% Secondly, we can use the first offset as the index and the second offset as the tag to store patterns, with their order inherently verified during the table lookup process. Consequently, both simplicity and compatibility are maintained.


% Using more subsequent accesses leads to an exponential increase in storage requirements. Meanwhile, utilizing the first two accesses can seamlessly integrate with recent hardware structures without introducing excessive additional control logic. Recent methods employ FT to filter out regions where only one block has been accessed. Therefore, we can capture the first two offsets of a candidate region when it is identified as not filtered out. Next, we consider how to index the stored patterns. The set-associative table first checks the index and then examines the tag, aligning perfectly with the temporal correlation between the first two accesses. Thus, we only need to use the first offset as the index and the second offset as the tag, concealing the temporal correlation within the matching process.
% Using more subsequent accesses actually leads to an exponential growth in storage requirements. Meanwhile, using the first two accesses can naturally {integrate with previous pattern index scheme} without introducing additional control logic.
% % As described in \S\ref{subsec:bit-pattern-based_prefetching}, when a region number hits in FT, which indicates that it has been activated once before, the current access is obviously the second access. So we can construct the search event at this point (\ding{202} in Fig.~\ref{fig:Gaze}b), without additional tracking buffer. 
% (detailed discussed in \S\ref{sec:design})
% From an implementation perspective, since the set-associative table logically first checks the index and then exams the tag, it perfectly aligns with the temporal correlation between the first two accesses. Thus, we only need to use the first offset as the index and the second offset as the tag, while the temporal correlation is hidden within the matching process.

% Using more subsequent accesses actually leads to an exponential growth in storage requirements. Meanwhile, using the first two accesses can naturally integrate with the recent hardware structure without introducing excessive additional control logic. Recent methods use FT to filter out the regions where there is only one block been accessed. Thus, we can capture the first two offsets of the candidate region when it is identified as not being filtered out. Next, we consider how to index the stored patterns. The set-associative table first checks the index and then examines the tag, which perfectly aligns with the temporal correlation between the first two accesses. Therefore, we only need to use the first offset as the index and the second offset as the tag, with the temporal correlation  is hidden within the matching process.

In addition, to maintain its high accuracy, Gaze employs a \textit{strict matching mechanism}, which prevents awakening prefetching when only one access matches while the other does not. This differs slightly from the mechanisms employed in Bingo~\cite{Bingo}, TAGE~\cite{TAGE}, and Domino~\cite{Domino}, which enable prediction even in cases of partial matches. We restrict this ability primarily because the temporal correlation between the first two accesses is a key characteristic.
However, we may miss prefetching opportunities when the candidate region fails to find a match, even though its upcoming pattern may be easy to follow. To compensate for this, we enhance the tracking structure with a {backup} prefetcher. The detail will be further discussed together with our dedicated two-stage aggressiveness control in \S\ref{subsec:Enhancement towards Spatial Streaming}.

% It is important to note that our {characterization} differs significantly from approaches that directly incorporate more {contexts} only from the trigger access, which is expensive and inefficient. For instance, PMP~\cite{PMP} uses \texttt{`Offset'}, so a 64-entry PHT is sufficient; SMS~\cite{SMS} additionally introduces PC (i.e., \texttt{`PC+Offset'}), necessitating as many as 16k entries (250× more) for optimal performance. As shown in Fig.~\ref{fig:sms_varying_offsets}, a 256-entry PHT suffices {for Gaze}.
% 我们认为，这是因为，作为pattern内部的特征，这种时间关联性更能从本质上特征化访问行为。
% 从设计上看，Gaze承接了先前数个方法，这保持了硬件简单性和可扩展性。
% We attribute this efficiency to the fact that the in-pattern temporal correlation represents some kind of internal features, making it more intrinsic in characterizing access patterns.
% Secondly, our method introduces a small amount of temporal information, empowering the prefetcher with the ability to identify some complex spatial patterns. This cannot be achieved by using trigger access alone.




==> texfile/5_des.tex <==
\subsection{Enhancement towards Spatial Streaming}
\label{subsec:Enhancement towards Spatial Streaming}
% 尽管spatial-pattern-based预取能够在多种场景里适用，但是其激进性在有些时候会过于高。
% memory-intensive 应用经常访问诸如矩阵、三维空间、结构体数组等的大型连续数据结构，它们大多是被连续分配的。访问存储了这些数据结构的区域通常产生被全部置位的空间模式。如果在其它区域应用这些访问模式，那么预取器可能将对区域内所有数据块发出请求。这是十分激进的，一个错误的预测将导致大量无用的预取请求。同时，因为这些请求是集中发出的，很可能会产生bad cache pollution，也会产生造成off-chip带宽上的瓶颈。
% 也就是说，我们需要针对这种访问行为的预取激进性进行控制。

% Streaming access is common in memory-intensive applications, as they often require loading large, contiguous data structures such as big matrices, 3D spaces, and arrays of structures.
% 这种访问行为通常会完整地加载数个区域。然而，这种访问行为被用于空间足迹预测则是非常激进的。


% Furthermore, we observe that the footprint generated by spatial streaming typically exhibit extremely high access density. As it indicates to prefetch almost the entire region, a misuse of this pattern can lead to severe over-prefetching. However, being overly conservative may miss numerous prefetching opportunities. To address this unique challenge, we further optimize Gaze with a dedicated two-stage approach to dynamically adjust the prefetch aggressiveness.
% At the same time, Gaze introduces a dedicated two-stage approach to mitigate the over-prefetching problem that often occurs in conventional schemes when they utilize high-dense footprints generated from spatial streaming
% 
% We enhance Gaze towards spatial streaming primarily due to the associated excessive aggressiveness.
Spatial streaming refers to the phenomenon of prolonged spatially-strided accessing~\cite{Primer}.
Despite the extensive research on spatial streaming over the past decades~\cite{stream1, stream2, stream3, stream4, stream5, stream6}, we still observe a unique unresolved challenge in utilizing its spatial footprints.
Specifically, we find that footprints generated by spatial streaming typically exhibit extremely high access density, especially when the stride is one, implying that when used for prefetching, speculative prefetches will be issued for almost all blocks in the candidate region.
Clearly, spatial streaming could greatly benefit from this high aggressiveness. However, in practice, various access patterns are often exhibited in an interleaved manner, and if such highly dense footprints are misused, the resulting massive and dense useless prefetches could cause significant cache pollution and off-chip bandwidth bottlenecks.
For example, Fig.~\ref{fig:ligra_bfs} provides the pseudocode of BFS-based graph processing algorithm in \texttt{Ligra}. The algorithm allocates a temporary space called \texttt{Frontier} to store sparsely distributed vertices to be processed in the current level. Thus, traversing \texttt{Frontier} (in function \texttt{BFS\_forward}) yields access patterns that include both irregular accessing and spatial streaming.
% Apparently, we have to eliminate the misuse of dense footprints.

% often incurs extremely high aggressiveness for spatial-pattern-based prefetching.
% Specifically, we find that footprints generated by spatial streaming typically exhibit extremely high access density. Prefetching based on this pattern would imply issuing speculative requests for almost all blocks within the candidate region.
% Consequently, even a single misuse could lead to massive and dense useless prefetches, causing significant cache pollution and off-chip bandwidth bottlenecks.
% Conversely, being overly conservative will result in numerous missed prefetching opportunities.


% We find that it typically produces highly dense accesses that exhibit a stride of one. In this common case, the resultant footprints are specific all-one bit-vectors.
% Streaming refers to a long sequence of strided accesses~\cite{Primer}. It has been extensively researched over the past decades~\cite{stream1, stream2, stream3, stream4, stream5, stream6}.
% Spatial streaming is a prevalent access behavior in memory-intensive programs, as they often need to load large, continuous data structures, such as big matrices, 3D spaces, and arrays of structures. 
% For example, Fig. \ref{fig:ligra_bfs} provides the pseudocode of BFS-based graph processing algorithm in \texttt{Ligra}. The algorithm allocates a temporary space called \texttt{Frontier} to store sparsely distributed vertices to be processed in the current level. Thus, traversing \texttt{Frontier} (in function \texttt{BFS\_forward}) yields access patterns that include spatial streaming.
% Although spatial streaming can be easily captured by spatial-pattern-based methods, we still observe a unique challenge. We find that it typically produces highly dense accesses that exhibit a stride of one. In this common case, the resultant footprints are specific all-one bit-vectors. Prefetching based on this pattern would imply issuing speculative requests for all blocks within the candidate region, which exhibits excessively high aggressiveness.
% Consequently, even a single misuse could lead to massive and dense useless prefetches, causing significant cache pollution and off-chip bandwidth bottlenecks.
% However, being overly conservative will result in numerous missed prefetching opportunities.
% A long sequence of strided accesses is referred to as a stream~\cite{Primer}.

\begin{figure}[tb]
    % \vspace{-15pt}
    \centering
    \includegraphics{figure/ligra_bfs_with_simple_example.pdf} % [width=0.45\textwidth]
    \caption{Pseudocode of BFS-based graph processing and an example of its illustration.}
    \label{fig:ligra_bfs}
    \vspace{-10pt}
\end{figure}

% To address the challenges of utilizing dense footprints in such complex access patterns,
To overcome this challenge, like many previous approaches{~\cite{stream2,stream3,stream4}}, we use a PC-based mechanism. Specifically, we deploy a Dense PC Table (DPCT) to record recent dense PCs, and a Dense Counter (DC) to track the frequency of recent dense footprints. We perform a double-checking using these two structures, and a two-stage approach to slowly increment the prefetch aggressiveness.

\textbf{Learning Phase.} Spatial streaming detection is illustrated in the upper part of Fig. \ref{fig:Gaze}a. When we finish tracking a region whose initial two accessed blocks are the block 0 and block 1 (i.e., \textit{r} in the figure), we check whether it is highly dense, i.e., whether all of its blocks have been accessed. If so, we record its trigger instruction into DPCT and increment the DC. Otherwise, we decrement DC, where a large value prompts a fast decrement.

\textbf{Prefetching Phase.} We employ a two-stage approach to adjust the prefetching aggressiveness when trying to apply this dense pattern to the candidate region.
In the first stage, for the candidate region, we detect the confidence level of exhibiting spatial streaming, and assign an initial prefetch aggressiveness accordingly. In the second stage, we dynamically adjust the prefetch aggressiveness based on subsequent accesses, gradually increasing it as needed.

\textit{Stage 1.} As shown in the upper part of Fig. \ref{fig:Gaze}c, when issuing prefetches for the region \textit{p} that is likely to be fully demanded by spatial streaming, if the trigger instruction has been recently labelled as a dense PC or DC is saturated, we assign a moderate level of aggressiveness: prefetching the first 16 blocks into the L1D and the remaining blocks into the L2C. We empirically set the number of initial blocks with higher aggressiveness to 16 (which is one-quarter of the region) to avoid losing prefetch opportunities while not being overly aggressive. Otherwise, if DC is half-saturated, indicating a lower probability that \textit{p} will be a dense region, we prefetch only the first 16 blocks into the L2C. If neither the trigger instruction has been labelled nor the DC is big enough, we refrain from prefetching. Meanwhile, when inserting this region into AT, we set the \texttt{stride\_flag} mark. This enables AT to prefetch the remaining blocks if the region exhibits streaming behavior later.

\textit{Stage 2.} AT will track all marked regions. For each one, we compute the two strides of the last three accesses. If the two strides both equal to one, we promote several subsequent blocks into the L1D (see the upper part of Fig.~\ref{fig:Gaze}c). The lower part of Fig. \ref{fig:Gaze}b shows how the PB merges the promotion pattern and the original prefetch pattern.

This stride-based approach can also serve as a {backup} predictor for cases where our strict matching mechanism (see \S\ref{subsec:Pattern Characterization}) fails to predict. As illustrated in the lower part of Fig.~\ref{fig:Gaze}c, if no match is found, the \texttt{stride\_flag} of this region is also set during tracking. Generally, for marked regions, once the last two strides match, the region-based stride prefetching is activated.

The differences between our region-based stride prefetching and other stride-based mechanisms are discussed below. Firstly, it serves a dual purpose: promoting aggressiveness and capturing potentially missed opportunities (\ding{208} in Fig. \ref{fig:Gaze}b). Secondly, it leverages the existing structure, e.g., the AT, and operates in a region rather than a global or per-PC view, avoiding the need for new tracking structures. 
% Thirdly, it just plays a secondary role. 
So, to maintain simplicity, complex scenarios such as multiple strides, are not handled.

% Accessing whole regions is common in memory-intensive applications, as they often require loading large, contiguous data structures such as big matrices, 3D spaces, and arrays of structures.
% However, prefetching a whole region is highly aggressive because an incorrect prediction can result in massive and concentrated useless prefetches. Additionally, these requests can further lead to bad cache pollution and off-chip bandwidth bottleneck.


% Even in scenarios with complex access patterns, a program may allocate contiguous temporary space to store frequently accessed data.
% For example, Fig.~\ref{fig:ligra_bfs} provides the pseudocode of BFS-based graph processing algorithm in \texttt{Ligra}~\cite{Ligra}.
% It allocates a temporary space called \texttt{Frontier} to store the sparsely distributed vertices to be processed in the current level.
% Traversing the \texttt{Frontier} (in function \texttt{BFS\_forward}) often generates spatial patterns indicating that the region is entirely demanded.

% However, prefetching a whole region is highly aggressive because an incorrect prediction can result in massive and concentrated useless prefetches. Additionally, these requests can further lead to bad cache pollution and off-chip bandwidth bottleneck.
% Being too conservative will result in numerous missed prefetching opportunities.
% Therefore, we specifically focus on how to balance prefetching aggressiveness in this case.



% For hardware prefetching, the incorrect usage of spatial patterns is unavoidable. But the resulting cost in this case is too expensive, so we specifically handle it.
% \textbf{Key innovation: two-stage aggressiveness control.}
% We enhance Gaze with this strategy to balance between the desire for the entire region and its possible massive negative effects.

% As shown in the example part of Fig.~\ref{fig:ligra_bfs}, when traversing all the neighbors of a ceratin vertex \textit{v} in the inner loop, two kinds of spatial patterns might be incorrectly employed. The first is the pattern generated by some other region of \textit{G}. This only results in few erroneous prefetches. The second is the pattern generated by the \textit{Frontier}, implying that the region needs to be entirely prefetched. However, the neighbors of \textit{v} are typically sparsely distributed, meaning that the other prefetched vertices are unlikely to be used. It can be seen that the consequences of the latter are fatal.
% These concentrated useless requests may further lead to bad cache pollution and create bottlenecks on off-chip bandwidth. 

% When the first two accessed blocks of a region are adjacent in space, the program may be loading contiguously stored data structure. When the data structure is small, the generated footprint of this region will exhibit a set segment. In contrast, when such the data structure is large, the program will probably load several regions consecutively, generating a series of spatial patterns where the first two accesses are blocks 0 and 1, with all bits set.

% Spatial streaming typically occurs during the traversal of large, contiguous data structures. 
% % 
% Identifying such behavior based on the first two accesses is straightforward. 
% When the first two accessed blocks of a region are adjacent in space, it suggests the program is loading a contiguous data structure. For smaller structures, the access footprint will exhibit a segment of set bits. In contrast, for large structures, the program will likely load several entire regions consecutively, generating a series of patterns where the first two accessed blocks are the block 0 and block 1.
% Moreover, these regions are often accessed in batches, generated by several identical instructions.

% Therefore, when a new region is initially activated and its first two accessed blocks are block 0 and block 1, we decide whether to prefetch the whole region based on the following criteria: we check if other recent regions are consistently entirely accessed (indicating that the program is likely accessing large contiguous data), or whether the trigger instruction of this region has entirely requested other regions recently (indicating a high probability of being a traversing instruction).
% In PHM, we use a counter named \textit{C} to indicate the frequency of recent whole-region accesses, and a tiny table named \textit{PCs} to store recent instructions that have triggered such behavior.
% % \textbf{Learning.} As shown in case 1 of Fig.~\ref{fig:Gaze}a, when we conclude the tracking of region \textit{r}{,} which is activated with block 0 and block 1 {being accessed first}, we check if the region is entirely demanded. If so, we record the trigger PC of \textit{r} into \textit{PCs} and increment the confidence counter \textit{C}. If not, we decrement \textit{C}, where a large value will lead to a fast decrement.

% \textbf{Learning.} As shown in case 1 of Fig.~\ref{fig:Gaze}a,
% {when we finish tracking a region that was initially accessed with block 0 and block 1 (i.e., \textit{r} in the figure),} we check if it is entirely demanded. If so, we record the trigger instruction of \textit{r} into \textit{PCs} and increment the confidence counter \textit{C}. If not, we decrement \textit{C}, where a large value will lead to a fast decrement.

% % As described in \S\ref{subsec:bit-pattern-based_prefetching}, any newly accessed region will be tracked by AT. Therefore, we can initially issue a small amount of prefetches instead of the whole region. Then we mark it in AT. AT will later decide whether to increase the aggressiveness. 

% \textbf{Prefetching.} We adjust the aggressiveness of prefetching in a two-stage manner when trying to prefetch all blocks of the candidate region: we start with a low initial aggressiveness (stage 1) and gradually increase it based on the subsequent access behavior (stage 2).

% \textbf{Stage 1.} As shown in case 1 of Fig.~\ref{fig:Gaze}c, when issuing prefetches for the region \textit{p} that is likely to be entirely demanded, if {its} trigger instruction has been encountered recently or the counter \textit{C} has saturated, {we assign a moderate level of aggressiveness: prefetching the first 16 blocks into L1D and the remaining blocks into L2C. If \textit{C} is only half saturated, indicating a lower probability that \textit{p} will be fully demanded,} we prefetch only the first 16 blocks into L2C. If neither the trigger instruction has been seen nor \textit{C} is big enough, we refrain from prefetching. Simultaneously, when inserting this region into AT, we set the \texttt{stride\_flag} mark. This allows AT to increase the aggressiveness later.

% \textbf{Stage 2.} {We track each \textit{marked} region within the AT.} For each one, we attempt to identify the strides of several recent accesses. If the stride is one and has maintained for a period, we increase aggressiveness by promoting several subsequent blocks into L1D. {We illustrate this aggressiveness promotion} in the lower part of Fig.~\ref{fig:Gaze}b: we ask the PB to merge the two prefetch patterns for the same region.

% The reason why we choose this stride-based method is that {it can also serve as a default predictor for cases where the \textit{strict matching mechanism} (see \S\ref{subsec:Pattern Index Scheme}) fails to predict. Since prefetching is triggered only if a matched pattern is found, we may miss prefetching opportunities when it fails to hit, even though the upcoming pattern may be easy to follow. To overcome this, we attempt to identify simple patterns exhibited within missed regions at a low cost.} As illustrated in case 2 of Fig.~\ref{fig:Gaze}c, if the event fails to hit, the \texttt{stride\_flag} of {this} region is also set during tracking. Generally, once the two strides generated from the last three accesses match and the \texttt{stride\_flag} is set, such region-based stride prefetching is activated.


% The differences between our region-based stride prefetching and other stride-based mechanisms are discussed below. Firstly, {it serves a dual purpose: promoting the aggressiveness and compensating for missed opportunities} (\ding{208} in Fig.~\ref{fig:Gaze}b). Secondly, it leverages the existing structure, i.e., AT, and works in a region view rather than in a global view or per-PC view, which would require new tracking structures. Thirdly, it only plays a secondary role. Thus, to maintain simplicity, we do not try to handle complicated scenarios.

\subsection{Pattern History Module}
\label{subsec:Pattern History Module}

As outlined in Fig.~\ref{fig:Gaze}b, in addition to the DPCT and DC, which are responsible for handling large spatial streaming mentioned in \S\ref{subsec:Enhancement towards Spatial Streaming} (denoted as case 1 for brevity), PHM also includes a Pattern History Table (PHT) used in typical scenarios (denoted as case 2). As previously mentioned, if the first two accesses to a region are spatially adjacent and occur at the head of the region, the DPCT and DC will learn this pattern. Otherwise, the PHT will be used to learn the pattern. Similarly, as for the footprint prediction of the candidate region, PHM invokes the corresponding structure based on its first two accessed blocks.
Additionally, PHT prefetches all blocks into the L1D.




% As shown in Fig.~\ref{fig:Gaze}, case 1 represents the scenario where the two-stage aggressiveness promotion needs to be employed, i.e., the region is activated with block 0 and 1 firstly been accessed, handled by \textit{PCs} and \textit{C}; case 2 represents the regular case managed by PHT. 

%     % continuous: 时间上连续重复某个动作
%     % contiguous: 物理连续，毗邻
%     % Continous is one thing that is on going. Consecutive is different things that happen in a row.

%     As shown in Fig.~\ref{fig:Gaze}, case 1 represents the scenario where the two-stage aggressiveness promotion needs to be employed, i.e., the region is activated with block 0 and 1 firstly been accessed, handled by \textit{PCs} and \textit{C}; case 2 represents the regular case managed by PHT. As depicted in Fig.~\ref{fig:Gaze}b, we deactivate a region when it becomes inactive: we stop the tracking and learn its spatial pattern.
%     Also, when a newly-activated region is accessed by another different demand, we use the event constructed by these two accesses, as well as the trigger PC to do prefetching (\ding{202}). 
%     Each entry in the AT is used to track an active region, where we introduce two additional 6-bit fields to store the offsets of the last two accesses to the region, which, together with the new access, will collectively calculate the two strides. AT decides whether to perform region-based stride prefetching (and aggressiveness promotion) based on whether the two strides match and the \texttt{stride\_flag} is set (\ding{203}).

% 如图所示，case 1 表示使用两阶段激进性提升的情况，即，区域被以第0块和第1块首先被访问来激活，由PCs和C负责；case 2 表示常规情况，由PHT负责。如图7b所示，当一个区域变成inactive的时候，我们结束对其的追踪并学习其访问模式；当inactive区域被两次不同的访问激活时，我们根据这两次访问的偏移构建事件，以寻找该区域可能展现的空间模式。AT的每个entry用于追踪一个active region。我们引入了两个额外的6-bit空间用以存储最近两次访问的偏移，它们和最新的访问共同计算两个stride。AT根据两个步长是否匹配，以及区域的stride_flag是否被置位来决定是否进行区域内基于步长的预取。

% As described in \S\ref{subsec:key_idea}, using one additional subsequent access introduces only a minor modifications to common bit-pattern-based prefetching control logic. However, it enables the prefetcher to gain the ability to eliminate these long-standing and increasingly prevalent mispredictions and overpredictions without sacrificing coverage.


% The overview of Gaze is illustrated in Fig.~\ref{fig:Gaze}a. Common bit-vector-based prefetchers extract the event from the trigger access, thus, PHT is probed for prefetching when the region number of an access address misses in both AT and FT (see \S\ref{subsec:bit-pattern-based_prefetching}). Although Gaze uses one more access to construct the event, it only introduces only minor modifications of control logic. As described in \S\ref{subsec:bit-pattern-based_prefetching}, when a region number hits in FT, which indicates that it has been accessed once before, the current one is evidently the second access. Thus, Gaze then uses these two accesses to form the event for prefetching (\ding{202}). 
% Gaze uses strict event matching mechanism to keep its efficiency: when an event misses in history table, Gaze do not attempt triggering prefetching with a similar but non-matching event. As a result, prefetching opportunities may be lost. To address this, we attempt to identify and leverage simple spatial regularities during the learning process with low overhead (\ding{203}).

% As shown in Fig.~\ref{fig:Gaze}, Pattern History Component (PHC) serves as the core of our proposal, \textit{simultaneously addressing mispredictions and overpredictions.} It is primarily comprised of Pattern History Table (PHT, used to handle common cases) and Contiguity-Aware Vector (CAVec, designed to handle the \textit{special} case). After separately describing how each of them functions (\S\ref{subsec:design_delayed_pattern} and \S\ref{subsec:cavec}), we then put these two together and present the processing flow of PHC (\S\ref{subsec:phc}). Subsequently, we introduce how the advanced AT compensates for potentially lost prefetch opportunities caused by the strict matching mechanism (\S\ref{subsec:design_simple_regularities}). Finally, in \S\ref{subsec:design_storage_requirements}, we present the storage overhead.


% We describe the organization of our Pattern History Table (PHT) in \S\ref{subsec:design_delayed_pattern}. In \S\ref{subsec:cavec}, we describe a special case and how we handle it. The cores of our proposal are \S\ref{subsec:design_delayed_pattern} and \S\ref{subsec:cavec}. In \S\ref{subsec:design_simple_regularities}, we explain how advanced AT identifies and leverages simple spatial regularities, and 


\subsection{Hardware Overhead}
\label{subsec:design_storage_requirements}
% TODO: here!!!
\textbf{Storage overhead.} Gaze sets the region size to 4KB (the same as a typical physical page). Table~\ref{tab:storage_requirements} presents the breakdown of each component and the total storage overhead. Both FT and AT have 64 entries, enabling the simultaneous tracking of 64 pages. PB uses 32 entries to store prefetch patterns for up to 32 pages, with four states for each offset: No Prefetch, Prefetch to L1D, L2C, and LLC (not used). PHT uses 4-way set-associativity. DPCT contains 8 entry. We omit the cost of DC since it only takes 3 bits.
Lastly, the total hardware overhead of Gaze is 4.46KB ($31\times$ lower than Bingo~\cite{Bingo}, 0.54KB less than PMP~\cite{PMP}, 1.91KB more than Berti~\cite{Berti}).
\begin{table}[htb]\renewcommand{\arraystretch}{1.5}
    \centering
    \caption{Detailed storage requi{re}ments}
    \label{tab:storage_requirements}
    % \vspace{-5pt}
    {
        \begin{tabular}{|p{0.45in}<{\centering}|p{2.05in}|p{0.4in}<{\centering}|}
            \hline
            \textbf{Structure}                   &
            \centering\textbf{Description}       &
            \textbf{Storage}                                         \\ \hline\hline

            FT                                   &
            \makecell[l]{\specialrule{0em}{0.5pt}{0.5pt}
            $8$-way; $64$ entries, each containing:                  \\
            $\bullet$ Region Tag ($36$b) \& LRU ($3$b)               \\
            $\bullet$ Hashed PC ($12$b) \& Trigger offset ($6$b)     \\
                \specialrule{0em}{0.5pt}{0.5pt}
            }                                    &
            456B                                                     \\ \hline

            AT                                   &
            \makecell[l]{\specialrule{0em}{0.5pt}{0.5pt}
            $8$-way; $64$ entries, each containing:                  \\
            $\bullet$ Region Tag ($36$b) \& LRU ($3$b)               \\
            $\bullet$ Hashed PC ($12$b) \& stride\_flag ($1$b)       \\
            $\bullet$ Trigger \& Second offset ($2\times6$b)         \\
            $\bullet$ Last \& Penultimate offset ($2\times6$b)       \\
            $\bullet$ Bit vector ($64$b)                             \\
                \specialrule{0em}{0.5pt}{0.5pt}
            }                                    &
            1128B                                                    \\ \hline

            PHT                                  &
            \makecell[l]{\specialrule{0em}{0.5pt}{0.5pt}
            $4$-way; $256$ entries, each containing:                 \\
            $\bullet$ Tag ($6$b) \& LRU ($2$b) \& Bit vector ($64$b) \\
                \specialrule{0em}{0.5pt}{0.5pt}
            }                                    &
            2304B                                                    \\ \hline

            DPCT                                 &
            \makecell[l]{\specialrule{0em}{0.5pt}{0.5pt}
            Fully-associative, $8$ entries, each containing:         \\
            $\bullet$ Hashed PC ($12$b) \& LRU ($3$b)                \\
                \specialrule{0em}{0.5pt}{0.5pt}
            }                                    &
            15B                                                      \\ \hline

            PB                                   &
            \makecell[l]{\specialrule{0em}{0.5pt}{0.5pt}
            $8$-way; $32$ entries, each containing:                  \\
            $\bullet$ Region Tag ($36$b) \& LRU ($3$b)               \\
            $\bullet$ Prefetch Pattern ($64\times 2$b)               \\
                \specialrule{0em}{0.5pt}{0.5pt}
            }                                    &
            668B                                                     \\ \hline \hline
            \multicolumn{2}{|c|}{\textbf{Total}} & \textbf{4.46KB}   \\ \hline
        \end{tabular}
        \vspace{-10pt}
    }
\end{table}

\textbf{Area and energy overhead.}
We estimate the area and access energy consumed by the pattern history module of Gaze (PHT and DPCT) and PMP (OPT and PPT) using CACTI~\cite{cacti1,cacti2} with its 22nm configuration. Gaze consumes about 29\% of the area compared to PMP (0.0034\thinspace  $mm^2$ vs. 0.0117\thinspace  $mm^2$). This is because each line in Gaze only costs 64b for storing a bit vector, where PMP costs 320b (160b) for storing a counter vector (coarse counter vector). Also, the read and write access to pattern history module of Gaze consumes less than 46\% of the energy required by PMP. Each table of Gaze can be accessed within a single CPU cycle.

The area and energy consumption of Gaze are much lower than that of Berti, as Berti extends each L1D line by 12 bits to accommodate fetch latency. This extension incurs an over $10\times$ increase in both area and access energy compared to PHM in Gaze.

% increasing the number of offsets may cause a poor timeliness and an unaffordable storage overhead. 

% However, increasing the number of offsets will exponentially expand the  event space size. At the same time, too many required observations can lead to poor timeliness, as prefetching will be delayed until we have fully observed the first few accesses. which can result in a exponentially enlarged event space size.

% HERE
% Despite this, we find that an ideal differentiation and timeliness can both be achieved by only additionally using the offset from the {\em second} access. Fig.~TODO shows the accuracy, coverage, and speedup of the SMS-like prefetcher with varying number of addresses that used for forming the event. The region size is set to 4KB (e.g. a physical page), so when only the trigger offset is used, the size of the history table is equal to the number of different offsets (i.e., 64). But when using two or more accesses, a full history table requires an unacceptable storage overhead and is inefficient. Therefore, we use a 256-entry\footnote{We evaluated the performance of the prefetcher with a 64, 128, 256, 512, and 1024-entry history table respectively, where the best performance is achieved when the table has 256 entries.} fully associative history table in these cases, which consumes less than 3KB. 

% As shown in Fig.~TODO, compared to SMS-Offset, using the first two offsets provides a 1\% improvement in IPC and a 15\% improvement in accuracy, with only a 2\% reduction in coverage. However, when the number of the used offsets increases again, a marginal gain in accuracy comes at a cost of a significant degradation in IPC and coverage. 
%is demonstrated.

% 使用256全连接表是一个不灵活的方案，因为它在硬件上较为复杂，并且可能会导致一些不太常用但又比较重要的模式被换出，从而造成较低的性能。

% In previous simple experiment we use a 256-entry fully associative table. However, in practice, this is not flexible as it is expensive in hardware, and even may lead to suboptimal overall performance. Moreover, due to locality, it is hard to have a large number of different patterns under the same trigger offset. Therefore, we adopt the trigger offset as the index and the second offset as the tag. This way, each set can differentiate multiple different patterns with the same trigger offset but different second offsets. Specifically, Gaze uses a 4-way set associative history table as shown in Fig.~\ref{fig:Gaze}b. The table is indexed by the trigger offset and is tagged by the second offset. 

% \subsection{Contiguity-Aware Vector}
% \label{subsec:cavec}
%     % The case
%     However, things do not turn out to be as straightforward as expected. Next, we discuss a \textit{special} case that occurs when the first two accesses to a certain region are the block 0 and block 1. For simplicity, below of this subsection may sometimes omit this premise or directly refer to the relevant patterns/regions as \textit{special} patterns/regions.

%     % Why we need to handle this
%     It is worth noting that when a large contiguous data structure, such as a large array, is accessed, the program often needs to entirely load multiple pages consecutively, leading to the generation of numerous consistent access patterns whose bits in the bit vector are all set {(contiguous accessing)}. In contrast, the program usually does not need to load several entire regions when not accessing such large data structures {(non-contiguous accessing)}. Since applications often involve a large number of such contiguous accesses, the patterns generated by contiguous accessing are prone to conflicts with those generated by non-contiguous accessing. 

%     % How do we handle this
%     To prevent, we do not store these discernible and often batch-occurring access patterns: 
%     {such contiguous accesses usually touch all blocks in sequence (which also means the first two accessed blocks are the block 0 and block 1).} So, we simply mark a pattern as produced by non-contiguous access if not all blocks are accessed. Therefore, for patterns starting with block 0 and block 1 firstly been accessed (\textit{special} patterns), we only store those whose bits are not all set into PHT (generated by non-contiguous accessing). 
%     But, when a new region comes, with the block 0 and block 1 firstly being accessed (\textit{special} region), how do we determine whether the region will be fully loaded {(contiguous accessing)} or will exhibit the stored access pattern {(non-contiguous accessing)}? It is easy to see that we need to decide whether the program is performing such contiguous accessing. We introduce the PC, which represents the program control flow information, and a \underline{C}ontiguity-\underline{A}ware \underline{Vec}tor (CAVec) to address this issue. 

%     Specifically, we record the \textit{special} access pattern, as well as the hashed PC (used as tag) into the PHT when non-contiguous accessing occurs (\ding{172}, where $\wedge b_i$ means the bitwise AND operation across all bits). 
%     And once a similar program context (i.e., the same hashed PC) and similar access behavior (i.e., the first two accesses are the block 0 and block 1) reappear, we utilize the corresponding access pattern to perform prefetching. 
%     Please note that we do not record the context information when the program exhibits such contiguous accessing. So, for those whose PC has not been encountered, there exists two possibilities: (1) it will be fully loaded because the program is accessing a large contiguous data structure that includes it; (2) it will exhibit another access pattern where not all blocks are accessed. We use CAVec to determine if the program is mainly exhibit contiguous accessing to decide whether to prefetch all blocks. 
%     % For regions where the PC has not been encountered, two possibilities exist: 1. it will be fully loaded because the program is loading a large contiguous data structure that includes it, or 2. It exhibits another pattern where not all blocks are accessed. We use CAVec to determine if the program is sequentially loading multiple pages to decide whether to prefetch all blocks. If it is more likely to exhibit another access pattern that does not match the patterns in the pattern table, we refrain from autonomously prefetching data blocks.

%     \begin{figure}[htb]
%         \centering
%         \includegraphics{figure/CAVec.pdf} % [width=0.45\textwidth]
%         \caption{Illustration of Contiguity-Aware Vector. The gray color indicates that the counter has reached its maximum/minimum value before this learning.}
%         \label{fig:CAVec}
%     \end{figure}

%     CAVec is composed of multiple (64 in default) counters as shown in Fig.~\ref{fig:CAVec}. For each block, CAVec employs a counter to track the times it has been loaded in the recent \textit{special} regions. Specifically, upon the arrival of a \textit{special} pattern, for each accessed block, the corresponding counter is incremented, up to a maximum of 8; otherwise, the corresponding counter is decremented, down to a minimum of 0. Prefetch pattern generated by CAVec is only a candidate and will be employed if the corresponding program context misses in the pattern table (\ding{177} in Fig.~\ref{fig:Gaze}). When recent \textit{special} regions are consistently loaded entirely, most counters are likely to be saturated. In contrast, when most counters are half-saturated (non-zero), it suggests that the program has recently alternated between two access behaviors. Therefore, we prefetch the blocks corresponding to saturated counters into L1D and those corresponding to half-saturated counters into L2C. Note that CAVec only responses for \textit{special} cases: it is only used to learn \textit{special} patterns, and to prefetch on \textit{special} regions.


%     \subsection{Integrating into PHC}
%     \label{subsec:phc}
%         In this section, we integrate the two basic components, PHT and CAVec, into PHC and present its processing flow, which includes elucidating how PHC learns access patterns and triggers prefetches.

%         {\bf Learning Phase:} 
%         When the accumulation of a certain region ends, i.e., the entry is evicted from the AT and sent to PHC, Gaze conducts an initial check to determine whether this pattern is a \textit{special} one (\ding{172}). 
%         The access pattern will be stored in two cases (\ding{173}): the pattern is a \textit{special} one and not all blocks are accessed (hashed PC is used as tag), or; the pattern is not a \textit{special} one (the second offset is used as tag). Additionally, CAVec will learn this pattern if it belongs to \textit{special} class (\ding{174}). Due to the existence of two types of tags (PC tag and $b_s$ tag) an extra bit in tag is used to indicate which one it belongs to. Besides, when storing a new pattern, if an entry with the same event already exists, PHC simply replaces its bit vector with the anchored new one and updates the LRU flag; otherwise the replacement based on LRU is used.

%         % The access pattern will be stored in two cases (\ding{173}): this pattern is a \textit{special} one and not all blocks are accessed (hashed PC is used as tag), or, this pattern is not a \textit{special} one (the second offset is used as tag). 
%         % If it is, the second offset is used as the tag is sent to CDT (\ding{203}). Subsequently, the first two offsets is used to construct the event. Next, CDT inserts this new entry: if an entry with the same event already exists, Gaze simply replaces its bit vector with the anchored new one and updates the LRU flag; otherwise the replacement based on LRU is used. On the other hand, if the first two offsets are adjacent, the entry is sent to FET (\ding{204}). {Each counter in the matched counter vector in incremented if the corresponding bit in the incoming bit vector is set.}

%         {\bf Prefetching Phase:} 
%         When an FT eviction occurs due to the arrival of the second different access to a certain region, PHC, as mentioned earlier, uses these first two offsets along with the hashed PC to find a history pattern which is likely to be replayed in this newly-accessed region.
%         PHC first extracts all candidate patterns, which include the set with the same trigger offset in pattern table and the contiguity-aware pattern from CAVec (\ding{175}). Subsequently, PHC builds the tag based on whether the region is a \textit{special} region (\ding{176}). It then employs this matching rule to select the prefetch pattern: if the region is not a \textit{special} one, a strict matching mechanism is applied; if the region is \textit{special}, the matched pattern is fetched if PC tag hits; otherwise, the contiguity-aware pattern is selected (\ding{177}). Finally, the prefetch pattern is sent to PB, ready for prefetching (\ding{178}).

%         % PHC first uses $b_f$ to fetch the set 
%         % first checks whether this region is a  (\ding{205}). If not, the trigger offset and the offset of the current access address (i.e., the second offset) are used together to search CDT (\ding{206}). If a hit is found, Gaze directly uses the stored bit vector as the prefetch pattern. If they are adjacent, {FET retrieves the matched counter vector and checks the frequency of each block. Only the blocks with a frequency exceeding a predefined threshold are prefetched (\ding{207}).}

%         % \textbf{Learning.} Specifically, whenever an access pattern arrives where the first two accessed blocks are the block 0 and block 1, we first update the CAVec:  for each set bit in the bit vector, the corresponding counter is incremented, up to a maximum of 8; for each unset bit, the corresponding counter is decremented, down to a minimum of 0. Then, we determine whether this pattern represents an entire-accessing, i.e., all bits are set. If it does, the pattern in fact has been perceived by CAVec, we do not store it. Otherwise, we use the hashed PC instead of the second offset as the tag to store it in set 0. Thus, an additional bit is used in the tag to indicate whether it stores the second offset or the hashed PC.

%         % \textbf{Prefetching.}
%         % When accessing such a new region, we first use the hashed PC as the tag to look up the set 0. If a hit occurs, which means that the instruction has been encountered before, we use this matched pattern for prefetching. Otherwise, we rely on the CAVec: all blocks corresponding to saturated counters are brought into L1D; and all blocks corresponding to non-zero counters are brought into L2C. When most counters of CAVec are half-saturated (non-zero), it indicates that the program has recently alternated between two access behaviors. To avoid losing prefetch opportunities and prevent excessive predictions, we bring the blocks corresponding to half-saturated counters into L2C (which, in practice, occurs very rarely).

%         % In addition to consecutive accessing, there are various other spatial patterns where the addresses of the second offsets are adjacent to the trigger ones. Examples include fetching data that spans several blocks, accessing with complex strides that start with one, or just taking those two data blocks. In other words, the possibility that they collide with each other is much higher than those patterns where the second offset is some distance away from the trigger one. This problem cannot be inherently solved by further increasing the number of observations. 
%         % % The authors of~\cite{DSPatch} and~\cite{PMP} find that patterns with a same event are similar with each other. 
%         % For these patterns, we try to extract their common features and prefetch those highly similar parts. 
%         % To avoid adding complexity, we adopt the method proposed in PMP~\cite{PMP} for similarity merging and extraction. Specifically, we implement another 64-entry direct mapped table called Feature Extraction Table (FET). Any case where the second offset is equal to the trigger plus or minus one\footnote{The two accesses may be out-of-ordered.}, i.e., they are consecutive, is served by FET. In FET, each entry employs a counter-vector to calculate the frequency of each block appearing in recent matched patterns. 

% % When the accumulation of a certain region ends, for each bit in the bit-vector, if set, the corresponding counter increases. with the trigger offset incrementing on each occurrence. When an event comprising two consecutive accesses arrives, the corresponding counter-vector from the table is fetched, and 

%         % \begin{figure}[htb]
%         %     \centering
%         %     \includegraphics{figure/PHTs.pdf} % [width=0.45\textwidth]
%         %     \caption{Hardware structure of CDC. For simplicity, the trigger offset is denoted as $b_t$, and $b_s$ is the offset from the second access.} 
%         %     \label{fig:PHTs}
%         % \end{figure}

% \subsection{Capturing Simple Spatial Regularities}
% \label{subsec:design_simple_regularities}

%     Since the use of an additional access plays a crucial role in differentiating conflicts and eliminating multiple inaccurate prefetches stemming from single-use regions, Gaze employs a strict matching mechanism. However, in common cases, when the second access fails to hit, some prefetch opportunities may be lost as pattern-based prefetching will not be issued. We notice that accesses to a certain region sometimes show a regularity that can be captured at a low cost during the accumulation in the AT. Specifically, we focus on capturing patterns that display a constant stride, as it is the most common regularity and can be implemented efficiently. Meanwhile, we can easily discard these redundant requests by checking whether the corresponding bit is set. 
%     % owing to the fact that the bit vector has recorded whether each block is accessed or not during the accumulation.


%     To capture stride patterns, we additionally use two 6-bit fields in each entry to record the offsets extracted from the the last two accesses which try to load an unrequested data block, respectively. Fig.~\ref{fig:AT} illustrates the structure of the modified AT. Each entry has four 6-bit fields named $b_t$, $b_s$, $b_l$ and $b_e$, respectively. Two of them ($b_l$ and $b_e$) are used to store offsts of the last two access, where $b_e$ is the earlier one, and the other two record the first two offsets denoted as $b_t$ (the trigger offset) and $b_s$ (the second offset), which will be used to form the event.\footnote{For the rest of the paper, unless specified, we use the same notations.}

%     \begin{figure}[htb]
%         \vspace{-3pt}
%         \centering
%         \includegraphics{figure/AT.pdf} % [width=0.45\textwidth]
%         \caption{Hardware structure of modified accumulation table. Among an entry, $b_l$ and $b_e$ are used to store offsts of the last two access, $b_t$ and $b_s$ are used to record the two offsets of the first two accesses.} 
%         \label{fig:AT}
%         \vspace{-5pt}
%     \end{figure}

%     First, let we suppose that the block address of the region start is $A$, the offset is $b$ and the block address of the requested data can be denoted as $B = A+b$. Each time a load request arrives and the region hits in AT, Gaze checks the stored bit vector to verify if this load is the first access to the requested data block. If the corresponding bit has not been set, the last two offsets, $b_l$ and $b_e$ are then used along with the current access offset $b$ to compute the two strides $d_1$ and $d_2$:
%     $
%         d_1 = b - b_l, d_2 = b_l - b_e.
%     $
%     If the two strides match (i.e., $d_1 = d_2 = d$) and this region has not triggered pattern-based prefetching before (StrideFlag, i.e., SF in the figure, is on), Gaze simply try to prefetch cachelines $B+ld$, $B+(l+1)d$, $\dots$, $B+(l+n)d$, where $l$ is the prefetch lookahead and $n$ is the stride prefetch degree. Besides, each request whose corresponding bit has been set or which exceeds the 4KB boundary will be discarded. Gaze finally updates the offsets of the last two accesses: 
%     $
%         b_e \gets b_l, b_l \gets b.
%     $ The default prefetch lookahead and degree are set to two and four, respectively.

%     We explain the difference between this and several previous methods: previous proposals often identify the strides between several addresses generated by a certain instruction, while Gaze utilizes the existing AT structure to capture the constant stride exhibited within a region. And, the purpose of this is merely to compensate for potentially lost prefetch opportunities at a low cost.

%     Although this stride prefetch seems to be suitable for handling cases where large contiguous data structures are accessed, we find that the expected performance is not achieved, as the effectiveness is compromised due to the out-of-order scheduling, the extended learning phase, and the limited prefetch lookahead and degree.
%     % To dynamically tune the prefetch degree, Gaze monitors the accuracy of the stride prefetching. Specifically, after every 32 feedbacks\footnote{If a request is served by a previously prefetched block, the number of useful prefetches is increased. Once an unused prefetched block is evicted, a feedback of useless prefetch is got.}, if the accuracy is greater than the higher threshold, the degree is increased up to eight, and if the accuracy is less than the lower one, the degree is decreased at least up to one, otherwise it remains. We empirically set the higher and the lower bound to 0.625 and 0.375, respectively. 


% \subsection{Putting All Together}


% Next we briefly introduce the learning phase and the prefetching phase of CDC.

% {\bf Learning Phase:} 
% When the accumulation of a certain region ends, i.e., the entry is evicted from the AT and sent to the two history tables, Gaze conducts an initial check to determine whether the first two offsets are adjacent (\ding{202}). If not, the entry is sent to CDT (\ding{203}). Subsequently, the first two offsets is used to construct the event. Next, CDT inserts this new entry: if an entry with the same event already exists, Gaze simply replaces its bit vector with the anchored new one and updates the LRU flag; otherwise the replacement based on LRU is used. On the other hand, if the first two offsets are adjacent, the entry is sent to FET (\ding{204}). {Each counter in the matched counter vector in incremented if the corresponding bit in the incoming bit vector is set.}

% {\bf Prefetching Phase:} 
% When an insertion of the AT occurs, that is, the second different access to a certain region arrives, Gaze, as mentioned earlier, first checks whether these two offsets are adjacent (\ding{205}). If not, the trigger offset and the offset of the current access address (i.e., the second offset) are used together to search CDT (\ding{206}). If a hit is found, Gaze directly uses the stored bit vector as the prefetch pattern. If they are adjacent, {FET retrieves the matched counter vector and checks the frequency of each block. Only the blocks with a frequency exceeding a predefined threshold are prefetched (\ding{207}).} Finally, the prefetch pattern is sent to PB for prefetching (\ding{208}).

% Unlike prediction mechanisms that use multiple events like Bingo~\cite{Bingo}, TAGE~\cite{TAGE} and Domino~\cite{Domino}, which can also make predictions when the multiple events are only partially matched, Gaze does not do pattern prefetching if only the trigger offset hits (which, in practice, always happens after working a while). These methods can be classified into two categories based on whether the event is completely arrived: the first category selects the sub-best-matching pattern when the event is fully arrived but no exact match is found, while the second class predicts the possible remaining part when the event is only partially arrived. First, as mentioned in Section~\ref{sec:motivation}, using the second offset can further distinguish conflicted patterns. If only the trigger offset is matched but the second is not, the actual access is likely to be different from the stored pattern. Second, prefetching the possible second accessed block when the trigger access arrives will be affected by the single-use regions. They all results in inaccurate prefetches. 


% \subsection{Storage Requirements}
% \label{subsec:design_storage_requirements}


% We believe that, considering its excellent performance benefits (see~\S\ref{sec:evaluation}), this overhead is acceptable. 
% Since working at L1D usually translates to higher performance, several L1D prefetchers have been proposed in recent years. However, due to the limited hardware complexity, the commercial community remains conservative about this. Our results show that Gaze can perform exceptionally well at both L1D and L2C, allowing it to be deployed more flexibly.

% Despite several L1D prefetchers have been proposed in recent years, the commercial community remains conservative due to the limited hardware complexity. 
% Although working at L1D usually translates to higher performance, our results show that Gaze can also perform exceptionally well at L2C, where a more complex prefetching mechanism .


% While our initial intention is to deploy Gaze at L1D for higher performance, our results also show that Gaze can perform exceptionally well at L2C with negligible accuracy loss, where hardware complexity is more tolerable.
% Therefore, we will demonstrate its outstanding performance when working at L2C, allowing for its application at the L2C level.

% We believe that this is acceptable because that the prefetcher proactively fetches data from remote main memory, which cannot be achieved by solely increasing cache size.

% \makegapedcells


==> texfile/6_metho.tex <==
\section{Evaluation}
\label{sec:methodology}

\subsection{Methodology}
\label{subsec:evaluation_methodology}

We evaluate Gaze along with other recent proposals using the ChampSim\footnote{Commit b4bfdb8. March 17, 2023.}~\cite{ChampSim}, a trace-driven cycle-accurate simulator capable of modeling various types of modern out-of-order processors.
ChampSim is an effective framework to study microarchitectural techniques.
This framework was used for the 1st instruction prefetching championship (IPC)~\cite{IPC1}, the 2nd and the 3rd data prefetching championships (DPC-2 and DPC-3)~\cite{DPC2, DPC3}, the 2nd cache replacement championship (CRC-2)~\cite{CRC2}, and ML-based data prefetching competition~\cite{ML-DPC}. Table~\ref{tab:simulator_configuration} presents the system configuration of our simulation.
%

\begin{table}[htbp]\renewcommand{\arraystretch}{1.5}
    % \vspace{-5pt}
    \centering
    \caption{Configuration of the simulator}
    \label{tab:simulator_configuration}
    % \vspace{-5pt}
    {
        \begin{tabularx}{3.2in}{m{0.35in} m{2.6in}}
            \hline
            \textbf{Core} & 1-8 cores, 4GHz, 4-wide OoO, 128/72-entry LQ/SQ, 352-entry ROB, hashed perceptron branch predictor \\
            \hline
            \textbf{TLBs} & ITLB/DTLB: 64-entry, {1 cycle}; STLB: 1536-entry, {8 cycles}                                       \\
            \hline
            \textbf{L1I}  & 32KB, 64B line, 8 way, 4 cycles, 8 MSHRs                                                           \\
            \hline
            \textbf{L1D}  & 48KB, 64B line, 12 way, 5 cycles, 16 MSHRs                                                         \\
            \hline
            \textbf{L2C}  & 512KB, 64B line, 8 way, 10 cycles, 32 MSHRs                                                        \\
            \hline
            \textbf{LLC}  & 2MB/core, 64B line, 16 way, 20 cycles, 64 MSHRs                                                    \\
            \hline
            \textbf{DRAM} & \textbf{1C}: Single channel, 1 rank/channel; \textbf{2C}: Dual channel, 1 rank/channel;
            \textbf{4C}: Dual channel, 2 ranks/channel;
            \textbf{8C}: Quad channel, 2 ranks/channel;\newline
            DDR4 \cite{ddr}, 8 banks/rank, 3200 MTPS, 64b data-bus, 2KB row buffer/bank,
            tRP = tRCD = tCAS = 12.5ns                                                                               \\
            \hline
        \end{tabularx}
    }
    % \vspace{-5pt}
\end{table}

\subsubsection{Workloads}
We use memory-intensive workloads that cover a variety of real-world applications for evaluation. Our evaluation traces are captured from \texttt{SPEC} \texttt{CPU2006}~\cite{SPEC06}, \texttt{SPEC CPU2017}~\cite{SPEC17}, \texttt{PARSEC 2.1}~\cite{PARSEC}, \texttt{Ligra}~\cite{Ligra} and \texttt{CloudSuite}~\cite{CloudSuite} benchmark suites. For \texttt{SPEC CPU2006} and \texttt{SPEC CPU2017} workloads, we use the instruction traces provided by DPC-2 and DPC-3. For \texttt{PARSEC 2.1} and \texttt{Ligra} workloads, we use the traces open-sourced by Pythia~\cite{Pythia} and Hermes~\cite{Hermes}. For \texttt{CloudSuite} workloads, we use the traces from the CRC-2. We only evaluate those traces that are memory-insensive among these workloads, i.e., traces that have at least one miss per kilo instructions (MPKI) at the LLC when without prefetching. Table~\ref{tab:evaluated_workloads} lists the number of traces for each suite, and some example workloads. In total, we evaluate 201 traces in our experiment.

\begin{table}[tb]\renewcommand{\arraystretch}{1.2}
    % \vspace{-5pt}
    \centering
    \caption{Evaluated workloads}
    \label{tab:evaluated_workloads}
    % \vspace{-5pt}
    {
        \begin{tabularx}{0.45\textwidth}{m{0.075\textwidth} c X}
            \toprule
            \textbf{Suite} & \textbf{\#Traces} & \textbf{Example Workloads}                \\
            \midrule
            SPEC06         & 39                & gcc, mcf, milc, soplex, sphinx3, leslie3d \\
            SPEC17         & 39                & gcc, mcf, bwaves, omnetpp, xalancbmk      \\
            Ligra          & 67                & pagerank, Bellman-ford, BFS, MIS          \\
            PARSEC         & 4                 & facesim, streamcluster                    \\
            Cloud          & 52                & nutch, cassandra, streaming               \\
            \bottomrule
        \end{tabularx}
    }
    \vspace{-10pt}
\end{table}


We use the first {200M} instructions to warmup, and the next 200M instructions to simulate per core. If a trace reaches its end before the simulator has executed enough instructions, it is replayed from the start. For multi-core simulations, any core that finishes early replays its trace until all cores have simulated enough instructions. We simulate both homogeneous and heterogeneous mixes in multi-core simulations. A homogeneous mix is composed of $n$ copies of a trace and a heterogeneous mix consists of $n$ randomly-selected traces, where $n$ is the number of cores. For $n$-core simulation, 201 homogeneous and $\lfloor\frac{201}{n}\rfloor$ heterogeneous mixes are evaluated. Each core runs one trace in the mix.



\subsubsection{Prefetchers}

In addition to Gaze, we evaluate seven state-of-the-art spatial prefetchers: SMS~\cite{SMS}, Bingo~\cite{Bingo}, DSPatch~\cite{DSPatch}, PMP~\cite{PMP}, IPCP~\cite{IPCP}, SPP-PPF~\cite{SPP, SPP-PPF} as well as Berti~\cite{Berti}.
The first four prefetchers are based on spaital pattern and have discussed in \S\ref{sec:background}.
IPCP is the latest composite prefetcher that attempts to capture multiple access patterns including Constant Stride, Complex Stride and Global Stream.
The last two prefetchers are based on delta-correlation~\cite{Primer}.
Berti is the latest delta-based prefetcher and can serve the highest L1D accuracy among all evaluated methods to the best of our knowledge. It takes into account the fetch latency to serve a timely and accurate prefetching. We evaluate enhanced Berti, namely vBerti, which works in virtual address and can generate cross-page prefetches.
The original vBerti allows for prefetching across up to 128 virtual pages (considering both forward and backward directions). However, based on our experiments, this configuration often results in significant performance degradation in multi-core environments {due to high fetch latencies, which prompts vBerti to select larger but less accurate deltas to keep timeliness}.
Thus, we restrict it to eight virtual pages (four per direction). This adjustment prevents the loss of prefetching opportunities while maintaining its high accuracy. 
Besides, we also evaluate the widely-used commercial prefetcher IP-stride~\cite{IP-stride}.


\begin{table}[tb]\renewcommand{\arraystretch}{1.2}
    \centering
    \caption{Configuration and storage overhead of evaluated proposals}
    \label{tab:prefetchers_configuration}
    % \vspace{-3pt}
    {
        \begin{tabularx}{3.4in}{m{0.45in} m{2.05in} m{0.4in}}
            \toprule
            SMS     & 2KB region, 64-entry FT/AT, \underline{16k-entry PHT}, \underline{32-entry PB}, \underline{fast access} & 116.6KB \\
            \midrule
            Bingo   & 2KB region, 64-entry FT/AT, \underline{16k-entry PHT}, \underline{32-entry PB}, \underline{fast access} & 138.6KB \\
            \midrule
            DSPatch & 2KB region, 64-entry PageBuffer, 256-entry SPT, \underline{32-entry PB}                                 & 4.25KB  \\
            \midrule
            PMP     & 4KB region, 64-entry FT/AT, 64-entry OPT, 32-entry PPT, 32-entry PB, MaxConf 32, L1/L2 Thresh 0.5/0.15  & 5.0KB   \\
            \midrule
            IPCP    & 64-entry IP table, 128-entry CSPT, 8-entry RST, 32-entry RR                                             & 0.7KB   \\
            \midrule
            SPP-PPF & Same configuration as in~\cite{SPP-PPF}                                                                 & 39.3KB  \\
            \midrule
            vBerti  & Virtual address, eight-page prefetch range                                                              & 2.55KB  \\
            \bottomrule
        \end{tabularx}
    }
    \vspace{-10pt}
\end{table}

For fairness, unless specified, all evaluated prefetchers are placed alone at \underline{L1D}. Each prefetcher is implemented based on its source code provided by the authors. The parameters and the storage overhead of all evaluated prefetchers is listed in Table~\ref{tab:prefetchers_configuration}, where the enhanced parts of SMS, Bingo and DSPatch are highlighted. For SMS and Bingo, we use 16k-entry PHTs for their optimal performance. However, an access to such huge PHT takes more than ten CPU cycles. This severely restricts their performance when deployed at L1D. Thus, we assume such an access can be completed within a single CPU cycle.
% 同时，我们不按照真实情况限制PHT的访问时间，假设它能在1个cpu周期内完成访问。
For DSPatch, we replace its out-of-dated Prefetch Buffer (PB). The PBs used in the four spatial-pattern-based methods as well as in Gaze have been fine-tuned and are uniform.
% Where the code come from? Table: parameters of them

\subsubsection{Main Metrics}
Below we list the metrics of interest with a brief introduction.

    {\bf Speedup.} The speedup is calculated as the ratio of IPC (instructions per cycle) achieved when with prefetching to that when without prefetching.

    {\bf Accuracy.} We use \textit{overall accuracy} rather than L1D accuracy. This is because some prefetchers choose to put blocks with lower-confidence into lower cache levels (e.g., L2C). These blocks \textit{cannot} be detected by L1D and thus will not be included in L1D accuracy by definition. However, they still play a crucial role in hiding long off-chip latencies and should therefore be considered.
All the evaluated methods do not put data into LLC. Assume that the number of useful and useless prefetched blocks at L1D are $n_a$ and $n_b$, respectively; the number of useful and useless prefetches at L2C are $m_a$ and $m_b$. Then the overall accuracy is $\frac{n_a + m_a}{n_a + n_b + m_a + m_b}$.
    % 我们使用总准确率而非L1D准确率。一些预取器能够将低置信度的数据预取进入更低的缓存层级，而这部分数据由于不会被L1D检测到，因此不会纳入L1D准确率的计算。但是这些预取进入低层级的数据也对隐藏长内存访问延时起到了关键作用，因此也应当纳入准确率的计算。
    % 由于所测量的预取器只将数据预取进入L1D和L2C，因此我们不用考虑LLC的预取块。这简化了计算。
    % 假设预取进入L1D数据块的数量是n，其中有用的请求有n_a个，预取进入L2C数据块的数量是m，其中有用的请求有m_a个。总准确率公式由下式给出。

    {\bf Coverage.}
The coverage refers to the ratio of demands that are successfully covered by prefetching.
% 覆盖率指预取成功覆盖了多少CPU demand
As off-chip misses mainly contribute to performance degradation, we evaluate the LLC coverage.
    % and L1D and L2C, due to their smaller capacities, tend to exhibit jitter in number of misses in the presence of prefetching

    {\bf Timeliness.} Since Gaze waits for an additional access, the timeliness may be impacted, i.e., there are more late prefetches. When a CPU access hits on an outstanding prefetch request, we say this prefetch is late~\cite{prefetch_throttling_3}. We measure the fraction of the late prefetches. A small fraction (e.g., 10\%) does not harm the performance, as they still save most of CPU cycles~\cite{prefetch_throttling_3}. % 因为Gaze额外等待了一次访问，因此可能会对及时性造成影响，即，产生较多晚的预取。When an demand access hits on an outstanding prefetch request, we say this prefetch is late.
% 我们测量late请求所占有效请求的比例。
% 少量late请求并不是致命的，因为它们仍然覆盖了一部分的延时~\cite{prefetch_throttling_3}。

% {\bf Cache pollution and bandwidth consumption.}
% Prefetchers with lower additional off-chip bandwidth consumption and fewer bad LLC pollution can better sustain performance when memory bandwidth utilization increases.
% For cache pollution, we specifically focus on the LLC pollution, as pollution in L1D and L2C has a relatively minor impact since the evicted data remains in the cache.
% We measure the number of polluted LLC blocks per {kilo} instructions caused by prefetching.\footnote{We use the same method as in~\cite{DSPatch} to quantify the bad LLC pollution caused by prefetching.}
% We use the number of off-chip requests (including demands and prefetches) to estimate the off-chip bandwidth.




==> texfile/7_eval.tex <==
\subsection{Results}
\label{sec:evaluation_results}

\subsubsection{Single-core Performance}
We measure the IPC improvement, accuracy, and coverage of all evaluated prefetchers on \texttt{SPEC06}, \texttt{SPEC17}, \texttt{Ligra}, \texttt{PARSEC} and \texttt{CloudSuite} benchmark suites. The results for each suite in single-core simulation are presented in the Fig.~\ref{fig:single_speedup},~\ref{fig:accuracy} and~\ref{fig:coverage}, respectively.
SMS, Bingo and DSPatch have been enhanced as described in \S\ref{sec:methodology}, enabling them to achieve their optimal performance when working at the L1D.

\begin{figure*}[tb]
    \centering
    \includegraphics[scale=1]{figure/single_speedup.pdf} % [width=0.45\textwidth]
    \caption{Speedup achieved by the {nine} evaluated prefetchers on each benchmark suite and the overall average (AVG). Group \texttt{f} and \texttt{c} means spatial-pattern-based prefethcers based on fine-grained events and coarse-grained events, respectively.}
    \label{fig:single_speedup}
    \vspace{-10pt}
\end{figure*}



{\bf Speedup.} Fig.~\ref{fig:single_speedup} presents the speedup achieved by all evaluated prefetchers in the single-core system, where group \texttt{f} and \texttt{c} means previous fine-grained and coarse-grained spatial-pattern-based prefethcers, respectively. As depicted in the figure, Gaze achieves the highest performance improvement across \underline{all} workload suites, with a notable {27.7\%} performance improvement over a no-prefetching baseline on average. Gaze outperforms the second-best prefetcher, Bingo, by {1.9\%}, and significantly surpasses the other two state-of-the-art prefetchers, PMP and vBerti, by {5.7\%} and {5.4\%} respectively. Furthermore, Gaze exhibits superior performance compared to DSPatch and SMS by {7.5\%} and {5.4\%}, and outperforms IPCP-L1, and SPP-PPF by {11.2\%} and {9.1\%}.

Only the two fine-grained prefetchers, Bingo and SMS, along with our novel Gaze, have demonstrated excellent performance (over 5\%) on scale-out \texttt{CloudSuite}, which is consists of server workloads. The other two coarse-grained spatial-pattern-based prefetchers, PMP and DSPatch, even result in performance degradation.\footnote{This is in line with the \texttt{CloudSuite} results mentioned in~\cite{PMP}.} Thus, their simple coarse-grained pattern characterization schemes are inefficient in this scenario.

The \texttt{Ligra} benchmark suite contains various graph algorithms, which involve numerous irregular accesses, as the neighbors of a certain vertex are typically distributed discretely. However, almost all prefetchers successfully achieve outstanding performance improvements on it. We believe that this is because \texttt{Ligra} is well-optimized for memory accessing.

\textbf{Accuracy.} Fig.~\ref{fig:accuracy} present the detailed prefetch accuracy of all evaluated prefetchers.
As shown in Fig.~\ref{fig:accuracy}, Gaze shows the second-highest prefetch accuracy among all prefetchers, surpassing SPP-PPF, IPCP-L1, SMS, Bingo, DSPatch and PMP by {73.6\%, 32.0\%, 4.7\%, 3.6\%, 37.6\%, and 22.5\%}, respectively. Surprisingly, compared to Bingo, where substantial hardware overhead is needed to fully utilize longer events \texttt{PC+Address} and \texttt{PC+Offset}, Gaze still outperforms it. This superiority can be attributed to its efficient pattern characterization ability.
% , which further takes into account footprint-internal temporal correlations.
It should be noted that the overall accuracy of vBerti is slightly lower than its L1D accuracy reported in~\cite{Berti}.\footnote{For vBerti, our evaluation also shows an L1D accuracy close to 90\%, which is in line with~\cite{Berti}.} This is because vBerti choose to prefetch low-confidence blocks into L2C, which the L1D cannot detect. Thus, the L1D accuracy does not include them.

Compared to the highly accurate vBerti, the accuracy of Gaze is only {4.2\%} lower when excluding \texttt{CloudSuite}. In contrast to other spatial prefetchers, vBerti and IP-stride exhibit excellent accuracy on \texttt{CloudSuite}, indicating that the access patterns of cloud workloads are strongly code-correlated. However, they only cover a small fraction of misses on it. For DSPatch, its second-order enhancement can offer accuracy-oriented prefetching when with only limited available bandwidth. However, the simple bitwise AND operation is insufficient to provide significant gains. Both PMP and Gaze are mainly based on \texttt{Offset}, yet Gaze achieves significantly higher accuracy compared to PMP. Although PMP expands the number of used historical patterns to 32, this does not fundamentally address the accuracy degradation caused by the flawed pattern characterization. In contrast, Gaze achieves a substantial accuracy improvement.

% Only vBerti exceeds Gaze by 11.7\% in accuracy, primarily on \texttt{CloudSuite}. However, Gaze outperforms Berti by 4.4\% if \texttt{CloudSuite} is not included. For DSPatch, its second-order enhancement can offer an accuracy-towarded prefetching when with only limited available bandwidth. However, the simple bitwise AND operation is insufficient to provide significant gains. Both PMP and Gaze are mainly based on \texttt{Offset}, yet Gaze achieves significantly higher accuracy compared to PMP. Although PMP expands the number of used historical patterns to 32, this does not fundamentally address the accuracy degradation caused by the flawed pattern characterization. In contrast, Gaze achieves a substantial accuracy improvement by only additionally leveraging the in-pattern temporal correlation.

% Berti的准确率略高于Gaze xx%，这是因为它在Cloud上取得了极高准确率。如果将CloudSuite排除，Gaze则在其它工作集上所取得的准确率高于Berti xx%。
% 对于DSPatch而言，其second-order enhancement能够针对低可用带宽场景进行优化，以相应提供准确率为导向的预取。但是，其简单地在两个最新模式进行与操作不足以提供高的性能提升。
% PMP和Gaze一样使用Offset作为事件，但是Gaze取得了远高于PMP的准确率。PMP 将所参考的历史模式的数量扩展到32个，但是这并不能从根本解决粗粒度事件带来的准确率降级问题。
% Gaze 只是通过额外使用前两次访问的时间关系，却能带来准确率的大幅提升。

% {Berti, PMP, and Gaze prefetch low-confidence data blocks into L2C, contributing to performance improvements. Therefore, for fairness, we additionally measure the L2C accuracy as well as the overall accuracy of these three prefetchers. As for L2C accuracy, only those blocks that are intentionally placed into L2C by the prefetcher are calculated, while blocks that are prefetched into L1D but have copies left in L2C are not considered. It is worth noting that the overall accuracy better characterizes these three prefetchers, as it includes the ratio of requests allocated to both L1D and L2C, in addition to L1D and L2C accuracy. As shown in Fig.~\ref{fig:overall_accuracy}, although Berti achieves the highest L1D accuracy, its L2C accuracy is relatively low. Additionally, Berti allocates nearly half of the prefetch requests to L2C, resulting in a lower overall accuracy, which is also why its performance falls short of expectations. PMP allocates nearly one-third of low-confidence requests to L2C, leading to an 8-percentage-point reduction in overall accuracy when considering these data blocks. The FET of Gaze can issue L2C prefetch requests, but the ratio is relatively low, and while L2C accuracy is the lowest, its overall accuracy is not significantly impacted. In summary, Gaze achieves the highest overall accuracy.}

\begin{figure}[tb]
    % \vspace{-12pt}
    \centering
    \includegraphics[scale=1]{figure/accuracy.pdf} % [width=0.45\textwidth]
    \caption{Prefetch accuracy of evaluated prefetchers on each benchmark suite and the overall average (AVG).}
    \label{fig:accuracy}
    \vspace{-10pt}
\end{figure}

% \begin{figure}[htb]
%     \centering
%     \includegraphics[scale=1]{figure/overall_accuracy.pdf} % [width=0.45\textwidth]
%     \caption{{Average L2C and overall accuracy of three main prefetchers.}}
%     \label{fig:overall_accuracy}
% \end{figure}

{\bf Coverage.} As shown in Fig.~\ref{fig:coverage}, Gaze achieves a moderate coverage, exceeding the highly accurate vBerti by {6.6\%}, and remaining at the same level as Bingo and PMP. Gaze achieves nearly no coverage penalty in spite of its strict matching mechanism, which avoids issuing prefetches when the event only partially matches. Gaze still exceeds DSPatch, which is capable of providing coverage-oriented prefetching, by {7.5\%}.
% (2.2\% and 0.4\% lower)
This shows that the eliminated prefetches of Gaze are almost entirely inaccurate. On top of that, vBerti fails to cover enough misses in \texttt{CloudSuite}, where its speedup falls below that of Gaze, Bingo and SMS.

\begin{figure}[htb]
    % \vspace{-10pt}
    \centering
    \includegraphics[scale=1]{figure/coverage.pdf} % [width=0.45\textwidth]
    \caption{LLC miss coverage and timeliness of evaluated prefetchers on each benchmark suite and the overall average (AVG). Each bar represents the covered portion, where the lower part stands for the late but useful.}
    \label{fig:coverage}
    \vspace{-10pt}
\end{figure}

{\bf Timeliness.}
% Across all traces, Gaze produces 18.4\% fewer late prefetches than Bingo produces (12.4\% vs. 15.2\%), and 12.7\% more than PMP and Berti (both have 11.0\%). IPCP-L1 and SPP-PPF show the worst timeliness.
As shown in Fig.~\ref{fig:coverage}, across all traces, Gaze achieves the second-best timeliness {(IP-stride is discarded)}. Gaze only incurs {0.5} percentage points more late prefetches than vBerti ({12.3\%} vs. {11.8\%}). However, vBerti achieves this by extending all L1D lines, all MSHRs, and all entries in Prefetch Queue (PQ) to compute fetch latencies. But this only brings marginal benefits since a small fraction does not harm performance~\cite{prefetch_throttling_3}. Compared to the other four spatial-pattern-based prefetchers, the additional enhancement of Gaze does not degrade the timeliness. We attribute this to its high accuracy, which allows accurate prefetches to be issued more quickly, minimizing the blocking effect of useless ones. IPCP-L1 and SPP-PPF demonstrate poor timeliness, which is unacceptable for high-performance prefetching.


% 在所有的工作集上，Berti的取得的时效性最好，这是因为其对L1D的数据、MSHR和PQ的每行进行了扩展，以计算拿取数据的时延。
% A small fraction (e.g., 10\%) does not harm the performance, as they still save most of CPU cycles~\cite{prefetch_throttling_3}.
% 相比于其它四个spatial-pattern-based 预取器，Gaze多等待一次访问并没有造成坏的时效性。我们认为，这是因为Gaze的高准确率让准确的预取能够更快地发出，尽量少地受到无效预取的阻塞。
% IPCP-L1和SPP-PPF展现了极差的时效性，这种对高性能预取而言是不可以接受的。


% 

% We take \texttt{Ligra} suite, which exhibits numerous complex access patterns that typically require complicated approaches to identify in previous methods, as an example to attempt to explain why, with a simple mechanism\textemdash by additionally using one subsequent access\textemdash Gaze can achieve such a significant performance improvement.
% \texttt{Ligra} suite contains several kinds of graph algorithms, such as \texttt{BFS}, \texttt{PageRank} and \texttt{Bellman-Ford}. These graph algorithms often utilize adjacency lists to represent the sparse graphs. In this way, all the vertices are usually stored in an array. But the edges of a certain vertex are likely to point to different regions. 
% 以区域视角而言，一个区域在激活时间内哪些节点被访问几乎是没有什么规律的。既不能直接迁移到其它区域上，也
% 尽管如此，其部分邻居可能位于同一内存区域，对它们的遍历将产生一些没有明显规律的空间模式。
% 如果只使用触发访问，无论使用细粒度的事件还是粗粒度的事件，我们都不能有效地利用这些空间模式。
% 


% 因为访问某节点的邻居是具有一定时间顺序的，
% 我们假设某一vertex为a，其在某一区域有部分邻居，b1又有邻居c
% 如果我们使用细粒度事件，例如PC+Address时，其再发生意味着区域又以b1又被访问了。但是，值得注意的是，这可能只是该邻居的邻居触发的，
%  making the utilization of the second address essential to effectively capture these access patterns.

% For example, on a \texttt{PageRank} trace in \texttt{Ligra}, Gaze achieves an accuracy of over 50\%, while bit-pattern-based prefetchers like PMP and Bingo, which only rely on trigger accesses to form events, only achieve 23\% and 19\%, respectively. Bingo utilize fine-grained event, but still struggles to handle these irregular access patterns. This observation indicates that although fine-grained events often imply a higher probability of replaying same access patterns in general cases, they still cannot address this problem effectively. However, by using the second offset, Gaze can significantly improve accuracy.

% Meanwhile, our results mostly corroborate previous works~\cite{Berti, Pythia, IPCP, DSPatch}, indicating that spatial prefetchers struggle to perform well in server applications such as \texttt{CloudSuite}. From the results it can be observed that, among the several methods we compared, only Bingo achieved a 3\% IPC improvement, and PMP even suffered significant performance degradation due to its low accuracy and high aggressiveness. The other methods show little to no noticeable performance improvement. However, Gaze successfully achieves an average IPC improvement of 7.5\% in these server applications. We believe that the requirement for one additional subsequent access of a region actually introduces a small temporal information at negligible cost. This small temporal information empowers Gaze with the ability to recognize some irregular patterns.

% As shown in Fig.~\ref{fig:single_speedup}, on \texttt{SPEC06}, \texttt{SPEC17} and \texttt{PARSEC}, Gaze achieves comparable performance with the aggressive PMP prefetcher, which significantly outperforms the other four methods.
% It can be expected that, with an increasing number of cores, memory bandwidth contention will intensify, favoring prefetchers with higher accuracy to sustain performance, whereas sacrificing accuracy for coverage may result in performance degradation (Fig.~\ref{fig:single_multi}). Moreover, as shown in Fig.~\ref{fig:coverage}, the two prefetchers employing fine-grained events (SMS and Bingo) exhibit the lowest coverage, as they can hardly issue prefetches for unseen regions and instructions, thereby missing numerous prefetch opportunities. 

% \begin{figure}[tb]
%     \vspace{-3pt}
%     \centering
%     \includegraphics[scale=1]{figure/rr_bwc_llcp.pdf} % [width=0.45\textwidth]
%     \caption{(a) Ratio of extra bandwidth consumption and (b) number of LLC pollution per kilo instructions (PKI) of evaluated prefetchers.}
%     \label{fig:redundant_pollution}
%     \vspace{-15pt}
% \end{figure}

% \textbf{LLC Pollution.}
% As shown in Fig.~\ref{fig:redundant_pollution}, we present the ratio of extra bandwidth consumption and the value of polluted LLC blocks per kilo instructions. Gaze achieves the highest performance improvement with the second-lowest extra bandwidth consumption and the fewest bad LLC pollution among all evaluated prefetchers. The extra bandwidth consumption of Gaze is even 23.4\% and 32.0\% lower than that of fine-grained SMS and Bingo. Coarse-grained PMP and DSPatch exhibit the highest additional bandwidth consumption, accounting for 32.8\% and 31.8\%. SPP-PPF, IPCP-L1 and Berti generate 20.6\%, 12.3\% and 6.9\% additional bandwidth consumption. Cache pollution exhibits similar characteristics to bandwidth consumption (Fig.~\ref{fig:redundant_pollution}b). It is noteworthy that about four percent of LLC misses are caused by cache pollution resulting from PMP, which we believe is not something that can be ignored further.



\subsubsection{{Performance Analysis}}
\label{subsubsec:performance_analysis}

% Gaze的性能提升可以归功于两个组件，即，PHT和PCs。PCs主要负责学习整页访问这种访问行为，而PHT负责其它常规情况。图10展现了在所有trace上各个组件的效用，以及它们的平均（标记在曲线结尾）。
% 在图中可以看见，PHT组件所带来的性能提升波动较小，因为大部分工作集的访问模式都能被PHT利用。而PCs组件所带来的性能提升波动较大，经常无法利用一些工作集的访问模式。尽管如此，PCs不会在这些工作集上带来负面收益，这是因为我们较为保守的初始激进性阻止了不合理的整页预取。
% 靠近左边的点表示它们在那些访问模式不容易利用的工作集上取得的效果。在这些工作集上，Gaze取得的性能提升和PHT所带来的几乎持平。
% 对于那些访问模式更容易利用的工作集而言，Gaze则将两者性能充分发挥。The more
% benefits achieved by Gaze mainly stem from the better
% utilization for two types of memory access patterns. Gaze既能够针对不同情况调用相关组件，并有效避免了过度激进带来的负面效益。

% 如同其它空间预取器一样，Gaze也不可避免地在少量工作集上造成性能下降。我们观测到了最高10%的性能下降，在201个traces里，where PMP和Berti最高带来了xx和xx的性能下降。因此，Gaze的性能波动是可接受的。

% Gaze specifically tunes the prefetch aggressiveness for streaming scenarios since naively relying on streaming patterns could cause dense useless prefetches in false-positive regions. 
% In particular, based on the behavior of the region's first two accesses, Gaze will redirect the potential streaming ones to the streaming module for fine-grained learning and prefetching.
% An alternative way would be to further enhance the pattern characterization by incorporating more initial accesses. However, we do not choose this because of the extra hardware complexity, the loss of prefetching opportunities and the interference from out-of-order scheduling. 
% , and the marginal gains (as illustrated in Fig.~\ref{fig:sms_varying_offsets}). Additionally, using more accesses may be ineffective due to interference from out-of-order execution and may not meet the timeliness requirements of other regular patterns.


% We do not choose to use more accesses to characterize access patterns, as this would bring extra complexity and yield only marginal benefits due to interference from out-of-order execution, loss of prefetching opportunities, and the timeliness requirements of other regular patterns.
% over-aggressiveness presented in conventional bit-pattern-based prefetchers. The dense patterns generated for prefetching in false-positive regions .
% In this part, we show the shortcomings of naively relying on the PHT to handle these dense regions in conventional methods and the benefits brought by fine-grained aggressiveness control.
% to significantly interfere with the Pattern History Table (PHT). 
% Employing patterns learned from Spatial Streaming in false-positive regions generates a large number of invalid requests, and the sparse patterns produced in false-positive regions can overwrite the true dense patterns of Spatial Streaming. This leads to insufficient coverage of requests in actual Spatial Streaming regions. 
% Using more accesses to characterize access patterns could resolve this issue, but due to interference from out-of-order execution, loss of prefetching opportunities, and the timeliness requirements of other regular patterns, this approach yields only marginal benefits (as shown in Figure 4). In our complete design, these regions are not handled by the PHT but are redirected to the DPCT and DC modules, which can more finely learn the access patterns of potential Spatial Streaming regions.

The performance improvement of Gaze can be attributed to two main factors: the efficient pattern characterization, which further aligns with temporal property of memory accessing, and the spatial-streaming-towarded fine-grained prefetching control.

\begin{figure}[b]
    \vspace{-10pt}
    \centering
    \includegraphics[scale=1]{figure/breakdown.pdf} % [width=0.45\textwidth]
    \caption{{Effect of our pattern characterization scheme. We present the speedup brought by the two characterization settings and the full Gaze across all traces.}} %Offset means using the trigger offset to characterize spatial patterns. Gaze-PHT represents using our characterization shceme, without the streaming module.
    \label{fig:breakdown}
    % \vspace{-20pt}
\end{figure}

{Fig.~\ref{fig:breakdown} shows the effect of our new characterization scheme. It plots the performance improvements brought by naively using the trigger offset (Offset), and by leveraging information from the first two accesses (Gaze-PHT), respectively. 
The speedup of full Gaze, i.e., the synergy of pattern characterization and optimized streaming prefetching, is also plotted. The averages are marked at the end of each curve.}

% 图9左侧是数据预取没能起到明显作用的工作负载。它们有些对数据miss不敏感，而有些则是包含了难以学习的复杂访问模式。同时，它们通常不包含容易识别的spatial streaming访问，因此，Gaze-PHT和Gaze几乎取得相似的性能。Gaze-PHT额外引入的时间关系帮助它更好地特征化访问模式，因此，在这些工作负载上能够利用一部分的复杂模式，从而带来性能提升。在这些工作负载上，触发offset则几乎无法准确特征化访问模式，因此带来了严重的性能下降。
% resulting in performance degradation.
% Meanwhile, since they generally do not exhibit streaming access, the performance brought by Gaze-PHT and full Gaze are similar. 
% This is because their access patterns are typically easier to learn. 
% Meanwhile, these workloads exhibit streaming access. As seen in the figure, after introducing fine-grained enhancements for spatial streaming, the performance improvements provided by Gaze become even more pronounced.
{The workloads on the left side of Fig.~\ref{fig:breakdown} exhibit minimal spatial regularities. 
Consequently, simply relying on the trigger offset is ineffective in characterizing their access behaviors, leading to significant pattern misuse.
In contrast, Gaze-PHT successfully captures some prefetch opportunities.
%  by incorporating an additional access.
On the right side, data prefetching brings noticeable performance improvements, as these workloads typically exhibit various spatial regularities, including spatial streaming. 
The gap between Offset and Gaze-PHT indicates that, in these regular workloads, waiting for accurate characterization does not miss prefetching opportunities but enhances gains. However, we can also see the underutilization of streaming behavior.}


\begin{figure}[tb]
    % \vspace{-20pt}
    \centering
    \includegraphics[scale=1]{figure/ss_effect.pdf} % [width=0.45\textwidth]
    \caption{{Effect of the streaming module. We evaluate the speedup brought by the two streaming settings and the full Gaze on several representative workloads.}} % PHT4SS represents naively using the PHT for spatial streaming access. SM4SS stands for using the streaming module.
    \label{fig:ss_effect}
    \vspace{-10pt}
\end{figure}

\begin{figure*}[b]
    % \vspace{-10pt}
    \centering
    \includegraphics[scale=1]{figure/speedup_across_different_workloads.pdf} % [width=0.45\textwidth]
    \caption{{Detailed speedup achieved by vBerti, PMP and Gaze on representative traces and the averages on different categories.}}
    \label{fig:speedup_across_different_workloads}
    % \vspace{-20pt}
\end{figure*}

{Fig.~\ref{fig:ss_effect} shows the effect of the streaming-towarded enhancement on several representative workloads. We evaluate two streaming settings, one that naively uses PHT for spatial streaming (PHT4SS) and the other that employs our dedicated streaming module (SM4SS), i.e., DPCT and DC.
To highlight the effectiveness on the streaming behavior, both only operate in streaming regions (i.e., whose initial two accessed blocks are the block 0 and block 1). The speedup of full Gaze is also plotted. 
% Both only operate in marked regions to highlight, while other regions are ignored. The speedup of full Gaze is also plotted.
}

{The left side shows the results on some individual workload traces while the right part shows the results on several \texttt{Ligra} workloads. Each plotted \texttt{Ligra} workload contains two representative traces: one from the initial phase (with smaller suffix numbers) and the other from the computing phase (with larger suffix numbers). During the initial phase, the program is likely preparing data and therefore mainly exhibits streaming behavior, which can be easily captured. Consequently, the performance of PHT4SS, SM4SS, and Gaze are nearly the same. In contrast, during the computing phase, as analyzed in \S\ref{subsec:Enhancement towards Spatial Streaming}, various access patterns co-exist. Thus, naively relying on PHT may misuse the dense pattern. Therefore, the finer-grained streaming module performs much better for streaming behavior. }


% SM4SS achieves about a 2\% higher speedup compared to PHT4SS, along with improvements in accuracy and coverage of 1\% and 2\%, respectively.
% In these computing traces, SM4SS achieves about a 2\% higher speedup compared to PHT4SS, along with improvements in accuracy and coverage of 1\% and 2\%, respectively.

% In \texttt{bwaves}, the performance improvements of PHT4SS and SM4SS are nearly identical but significantly lower than those achieved by Gaze, indicating that there are almost no false positive streaming regions in this trace. In other workloads, the presence of false positive regions allows SM4SS to achieve higher performance improvements compared to PHT4SS.

% After excluding a total of 89 traces that contain almost no streaming behavior or consist primarily of streaming accesses, SM4SS achieves approximately 2.5\% performance improvement over PHT4SS across all our workloads. If the performance improvement of SM4SS in a trace is less than 5\%, we consider that trace to have minimal streaming behavior (55 traces). Additionally, if the performance differences among PHT4SS, SM4SS, and Full Gaze are less than 1\%, it indicates that the trace consists almost entirely of streaming accesses (42 traces).


% 图9显示了我们的模式特征化在所有trace上的效果。我们评估了两种特征化设置，即，仅使用触发offset(offset)，以及leveraging the temporal correlation between the first two accesses（Gaze-PHT）。他们都被设置为在所有区域上工作，包括那些被标记为可能的streaming区域，而Gaze-PHT的streaming module被关闭。我们额外绘制出完整Gaze所带来的全额性能提升作为参考。它们取得的平均speedup被marked at the end of each curve.
% 数据预取在图9右侧的工作负载上带来了明显的性能提升。这是因为它们的访问模式通常容易识别。利用额外一次初始访问并没有让Gaze-PHT损失预取机会，相反地，它带来的高准确性进一步强化了性能提升。
% 同时，这些工作负载也包含spatial streaming行为，从图中可以看见，引入了针对spatial streaming的优化后，Gaze所带来的性能提升更为显著。After introducing fine-grained enhancement for spatial streaming

% 图9显示了naive design的效果（PHT only），优化机会（Spatial Streaming Only）和面向spatial streaming增强后的效果（Gaze）。
% It can be seen that most of memory intensive workloads contain streaming access. % 这说明我们的模式特征化能够有效地标记出潜在的streaming区域，同时，streaming module也能有效利用它们。
% Some workloads contain almost exclusively streaming access (e.g., \texttt{BC-4}, \texttt{MIS-5000}). The PHT can directly capture this simple access pattern. Therefore, the performance improvements achieved by the three settings are nearly the same.
% 尽管naive design取得的性能已经优于最新的两个方法约2%。
% However we can observe that the PHT is easily to be disturbed, % 导致了低于预期的性能. 
% After introducing fine-grained enhancement for spatial streaming, Gaze can correctly invoke streaming prefetching in appropriate regions. Consequently, both coverage and accuracy are improved (compared to the naive design, coverage and accuracy increase by 2\% and 3\% on average across all traces, respectively). 
% The only exception is \texttt{GemsFDTD-1491}. This is because all potential streaming regions are simply redirected. However most of them are sparse, causing a slient streaming prefethcing. Designing a smarter redirection could further improve the performance, which we leave for future work.



% 图10显示了Gaze针对spatial streaming的优化在一些代表性工作集上取得的性能提升。我们评估了两种spatial streaming设置，即，naively使用PHT（PHT4SS）和使用由DPCT和DC构成的Streaming module（SM4SS）。两者仅在被标记为可能的streaming区域上工作，常规区域被忽略。我们同样绘制出完整Gaze所带来的全额性能提升作为参考。
% 图10左侧显示了它们在数个从SPEC06，SPEC17，PARSEC和CloudSuite中选取的工作集上的效果。图10右侧显示了它们的在数个Ligra工作集上的效果。对于每个图中的Ligra图算法工作负载，我们挑选了两个代表性trace，分别来自工作负载的初始化阶段（后缀数字较小）以及计算阶段（后缀数字较大）。在初始化阶段里，这些工作负载很可能在准备数据集，因此几乎仅展现简单的Streaming的访问行为，它能够直接被PHT捕捉，因此，PHT4SS，SM4SS和Gaze所带来的性能提升几乎相同。在计算阶段，如在SecIII.C的分析，多种访问模式共存。因此，naively relying on the PHT can be easily disturbed。因此，SM对Streaming访问更细粒度的学习能够更好地规避假阳性区域带来的负面效益。在图中Ligra计算阶段的traces里，SM4SS相比于PHT4SS取得了约2%更高的speedup，同时，准确率和覆盖率也分别提高了1%和2%。
% 在图10左侧的bwaves负载上，PHT4SS和SM4SS所取得的性能提升几乎相同，但又显著低于Gaze所取得的，这表示在这个trace里几乎不存在假阳性streaming区域。在其它负载里，由于假阳性区域的存在，SM4SS相比于PHT4SS取得了更高的性能提升。
% 在我们所有工作负载上，排除总共89个几乎不包含Streaming行为，或者几乎只包含streaming访问的trace之后，SM4SS相比于PHT4SS取得了约2.5%的性能提升。如果一个trace里，SM4SS所取得的性能提升低于5%，我们认为这个trace几乎不包含Streaming行为（55个），同时，如果PHT4SS，SM4SS，Full Gaze三者的性能差异低于1%则意味着trace几乎只包含streaming访问（42个）。

% As illustrated in Fig.~\ref{fig:breakdown}, the blue curve represents using PHT to handle all cases, including potential streaming regions. The red curve represents the effect of streaming prefetching, provided by DPCT and DC. It represents the extent of streaming access within the workload. 
% The black curve is their combination, that is, redirecting all potential regions to DPCT and DC, while PHT handles other regular cases.


% Therefore, performing fine-grained handling specifically for this pattern can achieve considerable improvements on some workloads (as indicated by the red curve). 



% The performance improvement of Gaze can be contributed to two parts: the PHT, which handles common cases, and the DPCT and DC, which specifically target spatial streaming. Fig.~\ref{fig:breakdown} shows the utility of each across all traces, with the averages marked at the end of each curve. It can be observed that the majority of workloads exhibit spatial streaming, while a few workloads show little to no such behavior. However, the spatial streaming part does not yield negative benefits in these workloads, suggesting that it can effectively detect spatial streaming, which effectively prevents unreasonable whole-region prefetching.
% Besides, we can conclude that the increased benefits achieved by Gaze are mainly due to its ability to selectively invoke relevant components for different scenarios and can effectively avoid the negative impacts of excessive aggressiveness.

% Similar to other spatial prefetchers, Gaze causes performance declines in few of workloads. We observe performance decreases of up to 9.3\% across all traces, where PMP and vBerti result in maximum performance declines of 27.4\% and 8.5\%, respectively. Therefore, the performance variability of Gaze is reasonable.


% 除此之外，我们在PCs上限制预取激进性成功阻止了不合理的整页预取。我们使用该策略让整页预取被更多地应用在正确的区域上，而不是其它常规区域上。我们通过统计正确预测的数量和平均每个错误标记区域带来的无效预取数量展示这种限制的有效性。我们 run 50M instructions to warmup and collect the results in the next 50M instructions 来快速收集结果。

% Meanwhile, after applying the two-stage aggressiveness promotion, the proportion of correctly predicted whole-accessed regions (i.e., we correctly predict that the region will be fully demanded) increases from 70.0\% to 93.4\%, indicating an extremely high coverage of such contiguous access behaviors. Meanwhile, the average number of useless prefetches generated by a misused whole-fetch prediction decreases by 67.0\%, from 20.6 to 6.8. This means that the massive negative effects of such an incorrect prediction are significantly decreased.

% Therefore, here we analyze the benefits of tuning the aggressiveness of deploying the prefetch pattern which indicates to fetch the whole region. Since one of the goal is to avoid their misuse on common regions (which will not be entirely demanded). Therefore, we simply classify the patterns that represent a whole fetch as class \textit{a}, and the rest belong to class \textit{b}. In this analysis, we run 50M instructions to warmup and collect the results in the next 50M instructions. We only analyze traces where the two classes are mixed (with at least one class accounting for 20\% of the total). This is because if only one class predominantly exists, the probability of such a misuse is low.


% After applying the two-stage aggressiveness promotion, the proportion of correctly predicted \textit{a} regions (i.e., we correctly predict that the region will be fully demanded) increases from 70.0\% to 93.4\%, indicating an extremely high coverage of such contiguous access behaviors. Meanwhile, the average number of useless prefetches generated by a misused \textit{a} prefetch pattern decreases by 67.0\%, from 20.6 to 6.8. This means that the massive negative effects of such an incorrect prediction are significantly decreased.


\subsubsection{{Comparative Study}}

% 在图11中，我们列出Gaze和最新的两个预取器在一系列代表性工作集上取得的性能提升，以及在不同类型工作集下取得的平均值。
% Berti在一些访问模式特别容易利用的工作集上，如，leslie3d, bwaves_s和xalancbmk_s，取得的性能提升远低于PMP和Gaze所取得的。
% 我们认为，这可能是因为Berti只能选择一个最佳delta，无法进行多步预测，而PMP和Gaze能够一次性对区域的访问进行预测，因此抓住了更多的预取机会。同时，Berti追求极致的及时性，导致所选择的delta偏大，损失少量近距离数据块的预取机会。然而，适当比例的late prefetches不会带来性能下降，因为它们仍然覆盖了大部分的访问延迟。
% PMP能够良好地工作在访问模式较为简单的工作集上，然而，却在一部分访问模式复杂的工作集上，如，GemsFDTD，PageRank，cassandra，带来严重性能下降。这是因为PMP没有针对其较高的激进性进行有效限制，导致过多错误预测被发出。
% Gaze能够良好地工作大部分工作集上，既能够充分利用简单的访问模式，也能有效地工作在复杂工作集上。除此之外，Gaze在少量工作集上造成的性能下降也是轻微的。

We present the performance improvements achieved by Gaze and the two latest spatial prefetchers, PMP and vBerti, across several representative workload traces in Fig.~\ref{fig:speedup_across_different_workloads}.

Compared to PMP and Gaze, vBerti shows relatively lower performance gains in workloads where spatial streaming exists, such as \texttt{leslie3d}, \texttt{bwaves\_s}, and \texttt{xalancbmk\_s}.
% These workloads are characterized by prominent spatial streaming, which can be readily learned by vBerti.  contributing to its  performance lower-than-expected
We find that a key factor is the occurrence of redundant prefetches, where prefetch requests are issued for blocks already resident in the L1D.
Spatial-pattern-based prefetching effectively avoids them by awakening prefetching in newly activated regions. In contrast, vBerti cannot naturally perform such checks, leading to significant redundant prefetches when data are repeatedly accessed. These redundant requests occupy the PQ, only to be discarded when the L1D explicitly checks them. Although this only slightly increases queuing latency, the issuance of normal prefetches is severely hindered, as the PQ may become saturated more frequently.
% , leaving little room for new, potentially useful prefetches. 
To demonstrate its impact, we implement an oracle version of vBerti (Oracle\_vBerti) that can determine whether a requested block is already present in the L1D before issuing a prefetch. If the block is present, Oracle\_vBerti simply drops the prefetch request. On \texttt{bwaves\_s}, the achieved speedup increases from 2.12 to 2.65. However, this optimization is not a panacea. We also observe a small performance degradation (-4.2\%) on \texttt{GemsFDTD}. Our further analysis reveals that, in many cases, the elimination of redundant prefetches allows more low-confidence prefetch requests to be added into the PQ, leading to a decrease in prefetch accuracy. Overall, the lack of mechanism to handle redundant prefetches hinders its performance to some extent.
% This highlights the complex interplay between prefetching strategies and the importance of carefully evaluating the impact of optimizations on different workloads.
% 这些trace上主要展现spatial streaming，这能够被vBerti轻易学习。我们发现，vBerti所取得的性能低于预期的重要原因之一是冗余预取，即，对已经存在于L1D的块发出的预取。基于空间模式的预取能够有效避免发出冗余预取，因为预取在新激活的区域里触发。而vBerti不会对区域进行检查，当区域被短期被反复访问时，冗余预取便会产生。冗余预取请求会占据PQ，直到它被CPU显式地检查后才会被忽略。这只轻微地增加排队延迟，但是，会严重阻碍正常预取的加入。我们实现了一个oracle_vberti，它能够在尝试发出预取时就得知所请求的数据块是否已经存在于L1D，如果存在，则提前放弃预取请求。Oracle_vBerti在bwave_s上取得了甚至略微超过Gaze的性能提升。
% 然而，我们同时发现，这个优化并不是一劳永逸的，它在leslie3d带来了小幅性能下降。我们发现这是因为在冗余预取的消失让更多低置信度的数据块有机会被发出，从而导致预取准确率大幅降低。
% 因此，对vBerti而言，仍然需要针对冗余预取进行优化。

% This can be explained by the fact that programs
% often access some blocks repeatedly in a short time and
% only the first access to the data block triggers a miss.


% Berti limits its prediction depth to one, whereas PMP and Gaze can generate all prefetches of a region in a single prediction. Thus, in these workloads, PMP and Gaze can capture more prefetch opportunities.
% Additionally, Berti tends to choose a relatively large delta to keep its timeliness. As a result, nearby data blocks may be overlooked.
% However, a rational fraction (e.g., 10\%) of late prefetches does not harm the performance, as they still save most of CPU cycles.

PMP performs well on workloads with simple access patterns but causes significant performance declines on some workloads with complex access behaviors, such as \texttt{canneal}, \texttt{PageRank}, and \texttt{cassandra}. This can be attributed to that using the trigger offset alone can not accurately characterize access behavior. 
Meanwhile, PMP lacks control over the resulting high aggressiveness.
% , where a match pattern can almost always be found after working for a while.

As shown, Gaze efficiently leverages both simple and complex access patterns. Moreover, the performance degradation caused by Gaze on some irregular workloads (e.g., \texttt{cloud9} and \texttt{mcf\_s}) is slight.
We observe performance decreases of up to {6.9\%} across all traces, where PMP and vBerti result in maximum performance declines of {27.3\%} and {8.5\%}, respectively. 
Thus, the performance variability of Gaze is reasonable.
{Table~\ref{tab:prefetcher_comparison} summarizes the comparison of Gaze, vBerti, PMP and Bingo.}

\begin{table}[tb]  
    \centering  
    \caption{{Comparison of Prefetchers}}  
    \label{tab:prefetcher_comparison}  
    \begin{tabular}{|c|c|c|c|}  
        \hline  
            \textbf{Prefetcher} & 
                \makecell[c]{
                    \specialrule{0em}{0.5pt}{0.5pt}
                    \textbf{Hardware}\\\textbf{Cost}\\
                    \specialrule{0em}{0.5pt}{0.5pt}
                } 
            & 
            \makecell[c]{
                \specialrule{0em}{0.5pt}{0.5pt}
                \textbf{Simple Pattern}\\(e.g., streaming)\\
                \specialrule{0em}{0.5pt}{0.5pt}
            } 
            &
            \makecell[c]{
                \specialrule{0em}{0.5pt}{0.5pt}
                \textbf{Complex Pattern}\\(e.g., cloud)\\
                \specialrule{0em}{0.5pt}{0.5pt}
            } \\ 
        \hline  \hline
            \makecell[c]{
                \specialrule{0em}{0.5pt}{0.5pt}
                \textbf{Gaze} \\
                \specialrule{0em}{0.5pt}{0.5pt}
            }  & \ding{52} & \ding{52} & \ding{52} \\ 
        \hline  
            \textbf{vBerti}    & 
            \makecell[c]{
                \specialrule{0em}{0.5pt}{0.5pt}
                \ding{52} \\ \\
                \specialrule{0em}{0.5pt}{0.5pt}
            }
             & 
                \makecell[c]{
                    \specialrule{0em}{0.5pt}{0.5pt}
                    \halfcheck \\ Redun. req.\\
                    \specialrule{0em}{0.5pt}{0.5pt}
                } &
                \makecell[c]{
                    \specialrule{0em}{0.5pt}{0.5pt}
                    \halfcheck \\ Low cov.\\
                    \specialrule{0em}{0.5pt}{0.5pt}
                } 
                \\ 
        \hline  
            \textbf{PMP}       & 
            \makecell[c]{
                \specialrule{0em}{0.5pt}{0.5pt}
                \ding{52} \\ \\
                \specialrule{0em}{0.5pt}{0.5pt}
            } & 
            \makecell[c]{
                \specialrule{0em}{0.5pt}{0.5pt}
                \ding{52} \\ \\
                \specialrule{0em}{0.5pt}{0.5pt}
            } & 
                \makecell[c]{
                    \specialrule{0em}{0.5pt}{0.5pt}
                    \ding{56} \\ Low acc.\\
                    \specialrule{0em}{0.5pt}{0.5pt}
                } 
                \\ \hline  
            \makecell[c]{
                \specialrule{0em}{0.5pt}{0.5pt}
                \textbf{Bingo} \\
                \specialrule{0em}{0.5pt}{0.5pt}
            }       & \ding{56} & \ding{52} & \ding{52} \\ 
        \hline  
    \end{tabular}  
\end{table}  

{In \texttt{lbm}, all three main prefetchers achieve high accuracy (over 90\%) and cover more than one-third of LLC misses, yet still result in performance degradations. This can be contributed to increased queuing delays for CPU demands at the DRAM controller.
%  caused by dense prefetches, leading to high demand latency. 
In fact, some prefetches are issued too early. Thus, a feasible solution could be to prioritize CPU demands during bandwidth bottlenecks.
Meanwhile, Gaze also experiences slight performance declines due to insufficient accuracy in a few traces, such as \texttt{xalancbmk\_s}.
% , Gaze experience slight performance declines mainly due to insufficient accuracy. 
Since active regions are tracked by AT, Gaze can observe whether the prefetch pattern matches actual accesses. Based on this, Gaze can set confidence for each pair of initial offsets, and can reject low-confidence prefetch patterns. We have implemented similar control for streaming behavior in Gaze. The extensions for other patterns are leaved for future work.}
% The vBerti maintains accuracy in irregular traces by measuring the confidence of deltas. For Gaze,
% Overall, the performance variability of Gaze is reasonable.




\subsubsection{{GAP and QMM Performance}}

% 我们还测量了几个主要预取器在 a subset of GAP 图算法负载和来自 Qualcomm (QMM) 的企业负载上取得的效果。GAP is a framework for graph analytics, 它包含了常用的图算法，以及来自真实世界的数据集 [32]. QMM负载是由 Qualcomm 提供的来自企业的匿名工作负载。尽管具体的应用被匿名了，但包含system activity，使之更加符合真实场景。 QMM负载来自CVP-1的public traces，且被来自[81]的improved converter进行过格式转换。

{We further present the performance of the three major prefetchers on a subset of \texttt{GAP} workloads~\cite{GAP} and Qualcomm (\texttt{QMM}) industry workloads. \texttt{GAP} is a framework for graph analytics, similar to \texttt{Ligra}. 
% It contains several common graph algorithms along with real-world datasets. 
\texttt{QMM} contains numerous anonymized industry traces released by Qualcomm in the first Championship Value Prediction (CVP-1)~\cite{CVP1}. The \texttt{QMM}  traces we use are converted by~\cite{qmm_converter}.}

{Our evaluation on \texttt{GAP} contains three graph algorithms (\texttt{cc}, \texttt{pr}, and \texttt{tc}) on two real-world datasets (\texttt{twitter} and \texttt{web-sk-2005}). As depicted in Fig.~\ref{fig:gap_qmm}a, similar to \texttt{Ligra}, \texttt{GAP} is sensitive to data misses. Gaze and vBerti both achieve outstanding improvements. However, PMP shows severe performance decline on the irregular trace.
On average, Gaze surpasses vBerti and PMP by 1.3\% and 2.7\%, respectively.}
% 如图11所示，我们测量了预取器在三种常见图算法，即，PageRank, Connected Components和Triangle Counting，使用两个real-world graphs (twitter, web sk-2005)上分别取得的效果。从图11可以观察到，GAP和Ligra展现了相似的内存特征，即，对数据miss敏感，且包含很多可以利用的规则访问。
% Gaze和vBerti在GAP上的表现相近，都带来了可观的性能提升，同时也有效避免了在访问模式不容易利用的trace上带来性能下降。得益于其极高的激进性，PMP既体现出更高的性能提升，也体现出更严重的性能下降。

\begin{figure}[tb]
    % \vspace{-10pt}
    \centering
    \includegraphics[scale=1]{figure/gap_qmm.pdf} % [width=0.45\textwidth]
    \caption{Speedup achieved for (a) GAP and (b) QMM benchmark suites by vBerti, PMP and Gaze. QMM is further divided into server (left part) and client (right part) workloads.}
    \label{fig:gap_qmm}
    \vspace{-5pt}
\end{figure}

{The \texttt{QMM} workloads can be furthre divided into two categories: server workloads (plotted on the left part of Fig.~\ref{fig:gap_qmm}b), which typically include large code footprints, and client workloads (plotted on the right part), which primarily consist of memory-intensive computing tasks. As shown, spatial prefetching achieves substantial performance improvements on client workloads but nearly on improvements on server workloads. This is because the primary bottleneck for \texttt{QMM} server workloads is instruction misses instead of data misses~\cite{Morrigan}. They have relatively higher L1I MPKI values and lower LLC MPKI values, compared to \texttt{CloudSuite}, which means that they are much less sensitive to data misses.
% Additionally, the irregular access patterns further limit the performance. 
In \texttt{QMM} server workloads, although Gaze successfully covers nearly one-third of the LLC misses, a slight decline is still observed (-1.6\% on average). Highly accurate vBerti also fails to provide effective gains (+0.4\%), while PMP brings significant performance drop (-10.2\%).}
% Compared to \texttt{QMM} server workloads, \texttt{CloudSuite} server workloads shows a  higher LLC MPKI and a lower L1I MPKI. 

% QMM 负载可以分为两类，即，client workloads and server workloads. client workloads主要包括浮点数和整数的计算负载；而server workloads则包含大量的code footprints以及不规则访问。从图11可以看到，对于QMM，数据预取器在Client工作集上取得了可观的性能提升，其中，vBerti，PMP和Gaze分别取得了6%，10%和11%的speedup。然而，数据预取在Server工作集上几乎不起作用。我们发现，不同于主要包含计算任务的client工作集，服务器工作集的主要性能瓶颈是指令miss。与此同时。大部分服务器工作集的LLC MPKI低于2，意味着它们 are much less sensitive to data miss, 以至于乱序处理就能够cover大部分的miss latency。
% 在具有这种特征的工作集里，主要目标为覆盖长的off-chip latency的数据预取器很难起到效果。此外这些工作集中的不规则访问进一步限制了空间预取器的性能。
% 在server workloads上，相比于vBerti，Gaze覆盖了更多的LLC miss，但预取准确率较低。尽管成功覆盖了约三分之一的miss，但因为这些工作集对数据miss不敏感，Gaze反而造成了轻微的性能下降（-1.6%）。高准确的vBerti也没有提供有效的性能提升（+0.4%）。PMP低效的模式特征化导致其很容易误用访问模式，因此造成了严重的性能下降(-10.2%)。
% Gaze和vBerti良好的准确率和预取激进性控制使得它们可以混合访问模式的工作集上。
% 可以注意到的是，数据预取器在QMM Server上取得的效果和在CloudSuite上取得的效果有很大差别。我们认为主要原因是 1. CloudSuite对数据miss更加敏感，它拥有相对更高LLC MPKI的以及更低的L1I MPKI。2. CloudSuite展现的访问模式更具有空间特征，数个空间预取器都在上面取得了更高的准确率和覆盖率。

\subsubsection{Multi-level Prefetching}

We evaluate eight combinations of several state-of-the-art prefetchers (Group 1). We also present their performance when combined with the current commercial L1D prefetcher IP-stride (Group 2).
Fig.~\ref{fig:multi_level_prefetching} shows the speedup achieved by these combinations.
%  compared to a system without prefetching.


\begin{figure}[b]
    \vspace{-5pt}
    \centering
    \includegraphics[scale=1]{figure/multi_level_prefetching.pdf} % [width=0.45\textwidth]
    \caption{Speedup achieved in multi-level prefetching. Group 1 contains the eight combinations of recent prefetchers. Group 2 shows their performance when combined with IP-stride.}
    \label{fig:multi_level_prefetching}
    % \vspace{-10pt}
\end{figure}

% As shown, due to the use of an L2 prefetcher, the LLC coverage is much higher (17.2\% higher on average), and thus more extra bandwidth is consumed (116.4\% more on average). However, despite eliminating more misses, only negligible or even negative impacts are observed. This further highlights the marginal benefits of improving coverage. 

% The combination Gaze+Bingo achieves the best performance improvement, with an increase of 0.04\% in IPC compared to only using Gaze at L1D. The other {nine} combinations still fall short of using Gaze alone.
% We believe Gaze has almost maximized the utilization of spatial regularities. Thus, employing additional spatial prefetchers only yields marginal benefits. The combinations that contain PMP fail to give performance improvements due to its over-aggressiveness. Berti achieves performance gains when working with these two L2C prefetchers, which indicates that its performance can be further enhanced.
% Given the extra hardware overhead and limited benefits, we believe that using Gaze alone at L1D is a better choice. Furthermore, when combined with the current commercial L1D prefetcher IP-stride, Gaze still achieves the best performance.

The combination Gaze+Bingo achieves the best performance improvement, with an increase of {0.34\%} in IPC compared to only using Gaze at L1D. The other nine combinations still fall short of using Gaze alone.
Bingo, PMP, DSPatch and Gaze all are bit-pattern-based. Consequently, they can act as filters when working together with Bingo, resulting in marginal performance improvements. In fact, performance degradations are even observed in several combinations due to the additional aggressiveness introduced by L2 prefetching. Delta-correlated vBerti shows room for performance enhancement when integrated with spatial-pattern-based Bingo.
Meanwhile, we do not see significant improvements when combining them with SPP-PPF.

When combined with the commercial L1D prefetcher IP-stride, Gaze still achieves the best performance. The vBerti is highly dependent on the completeness of access sequences, which can be a limitation when operating at the L2C.
%, working in conjunction with IP-stride.
{Likewise, when Gaze is deployed at L2C alongside an aggressive L1D prefetcher capable of generating cross-page prefetching, the true initial accesses may be difficult to obtain. In this case, similar to IPCP~\cite{IPCP}, transmitting metadata through MSHRs is a feasible solution. However, as we do not see any considerable benefit from multi-level prefetching, using Gaze alone at L1D is a better choice.}
% Given the extra hardware overhead and limited benefits, we believe that using Gaze alone at L1D is a better choice.
% 当Gaze被部署在L2C和一个激进的能够跨页预取的L1D预取器共同工作时，Gaze很可能难以观测到的区域的真实初始访问。在这个情况下，Gaze需要像IPCP一样依靠上层将元数据通过MSHR传输下来。不过，as we do not see any considerable benefit, 我们建议Gaze单独部署在L1D上。

\begin{figure}[tb]
    % \vspace{-10pt}
    \centering
    \includegraphics[scale=1]{figure/multi_core_performance.pdf} % [width=0.45\textwidth]
    \caption{Multi-core performance achieved in (a) homogeneous and (b) heterogeneous mixes.}
    \label{fig:multi_core}
    \vspace{-10pt}
\end{figure}
\subsubsection{Multi-core Performance}


Fig.~\ref{fig:multi_core} depicts the performance improvements in homogeneous and heterogeneous multi-core simulations. Thanks to the higher accuracy, the performance degradation of Gaze is more gradual. Gaze consistently achieves the highest performance across 1-8 cores. 
The two aggressive coarse-grained prefetchers, DSPatch and PMP, exhibit significantly performance degradation. The vBerti shows a relatively smoother degradation compared to PMP, DSPatch and SPP-PPF.
Thus, among all prefetchers, Gaze can be applied in a wider range of systems, delivering excellent performance both in scenarios with abundant memory bandwidth resources and higher bandwidth contention.


{We first focus on homogeneous results (Fig.~\ref{fig:multi_core}a) since the heterogeneous mixes involve interactions among different workloads. 
As the number of cores increases, bandwidth contention intensifies. 
Thanks to the higher accuracy, the degradation trends of Gaze, Bingo, and vBerti are more gradual. However, for PMP, the performance degradation becomes particularly severe when the number of cores increases to four or more. This is due to its inefficient characterization and excessive aggressiveness.
In eight-core homogeneous mixes, Gaze outperforms Bingo, PMP, and vBerti by 3.1\%, 11.7\%, and 9.0\%, respectively.}%  to isolate the impact of system resources in multi-core systems.
% The additional bandwidth consumption caused by prefetching exacerbates this contention, thereby reducing performance improvements. 
% , and by 1.9\%, 9.4\%, and 7.8\% in heterogeneous mixes.


\begin{table}[h]\renewcommand{\arraystretch}{1.5}
    % \vspace{-5pt}
    \centering
    \caption{{Selected four-core mixes}}
    \label{tab:mixes}
    % \vspace{-5pt}
    {
        \begin{tabularx}{3.1in}{m{0.2in} m{2.85in}}
            \hline
            \textbf{Mix1} & wrf-1254, Triangle-1, lbm\_s-2676, Triangle-6 \\
            \hline
            \textbf{Mix2} & GemsFDTD-1211, PageRank-19, BFS.B-5, BFS-5                                       \\
            \hline
            \textbf{Mix3}  & bwaves\_s-2609, BFSCC-1, wrf\_s-8065, astar-359                                                           \\
            \hline
            \textbf{Mix4}  & PageRank.D-24, bwaves-1963, PageRank-61, facesim-22                                                         \\
            \hline
            \textbf{Mix5}  & cass.-p0c0, cass.-p0c1, cass.-p0c2, cass.-p0c3                                                  \\
            \hline
        \end{tabularx}
    }
    % \vspace{-5pt}
\end{table}


{For heterogeneous simulations, we plot the prefetching performance on several representative four-core mixes (listed Table~\ref{tab:mixes}). As illustrated in Fig.~\ref{fig:multi_core_detail}, Gaze shows advantages in both per-core performance and the overall average.
It is noteworthy that, within a mix, the effectiveness of prefetching varies significantly across different cores. This can be attributed to the fact that heterogeneous workloads compete for shared resources  
in different manners. As a result, weaker workloads may struggle to secure sufficient resources, which can be further exacerbated in the presence of prefetching.
Some approaches attempt to introduce global control at the LLC to address this issue~\cite{prefetch_throttling_1,prefetch_throttling_2,prefetch_throttling_3}.
In eight-core heterogeneous mixes, Gaze outperforms  PMP and vBerti by 9.4\% and 7.8\%, respectively.}
% such as LLC, memory bandwidth, and DRAM 
% , and by  in heterogeneous mixes.

% 例如，在混合2中，vBerti在核心1和2工作地十分出色，但也因此导致核心0和核心3得不到足够的共享资源。

\begin{figure}[tb]
    % \vspace{-10pt}
    \centering
    \includegraphics[scale=1]{figure/multi_detail.pdf} % [width=0.45\textwidth]
    \caption{{Four-core performance achieved in different mixes.}}
    \label{fig:multi_core_detail}
    \vspace{-10pt}
\end{figure}


% 因为异构混合还包含了不同workload之间的影响，因此我们主要分析同构混合，以突出多核系统下系统资源的影响。在多核系统中，随着核心数量的增加，带宽争用加剧。而预取产生的额外带宽消耗会加剧争用。因此，性能提升下降。Gaze，Bingo和vBerti性能下降的趋势几乎相同。同时，它们拥有较高的准确率，因此，遭受的性能下降也就平缓。而PMP在核心数增加到4个及以上时，其性能下降尤为严重。这是因为PMP的低效特征化和过度激进性导致的过多的错误预测占据了更多的带宽。
% 在八核系统中，Gaze超过Bingo，vBerti和PMP分别3.1%，11.7%和 9.0% 在同构混合中，分别 1.9%, 9.4% 和 7.8% 在异构混合中。这表明Gaze在多核系统中的性能优势。

% {We further study the impact of mixes with different MPKI compositions on performance. We label combinations with both low MPKI traces as group L, both medium as group M, both high as group H, and one with low while the other with high as group LH. Within the LH group, the trace set with low/high MPKI is marked as LH\_L/LH\_H. We conduct this on a 2-core simulation as it is easier to observe and identify such the interactions.}

% {As shown in Fig.~\ref{fig:multi_core}b, Gaze achieves the highest average performance improvement across four groups: L, M, H, and LH. We can observe that the performance of the other three bit-pattern-based prefetchers, particularly PMP, significantly decrease as MPKI increases, especially when MPKI is high. This decrease is due to the growing demand for memory bandwidth, leading to reduced tolerance for inaccurate prefetches. These three bit-pattern-based prefetchers exhibit a higher proportion of inaccurate prefetches due to conflicts and single-use regions. The over-aggressive IPCP yields negative effects when at high MPKI levels. While Berti has lower overall accuracy and coverage than Gaze, its performance is more stable due to its lower aggressiveness and minimal extra bandwidth consumption.}

% {When two applications, one with low MPKI and the other with high MPKI, are combined, they influence performance by competing for shared LLC and memory bandwidth. Typically, applications with low MPKI can issue more memory requests, which triggering the prefetcher more frequently because their memory requests complete more quickly. Consequently, when combined with high MPKI applications, the contention for shared LLC and bandwidth increases. From the figure we can see that nearly all prefetchers accelerate low MPKI applications. However, on high MPKI applications, PMP and IPCP exhibit significant negative effects, While the benefits of SMS, Bingo, and Gaze are offset by their aggressiveness. Berti, with the lowest aggressiveness, provides reasonable acceleration for both.}

% {As prefetchers on different cores cannot communicate, we consider that this can be addressed to some extent by introducing a filter at the LLC. We leave this for future work. Balancing aggressiveness allows prefetchers to cover more misses, and Gaze maintains a certain level of aggressiveness while providing the highest overall accuracy.}


\begin{figure}[b]
    \vspace{-5pt}
    \centering
    \includegraphics[scale=1]{figure/dram_llc_l2c.pdf} % [width=0.45\textwidth]
    \caption{Sensitivity to (a) DRAM bandwidth, (b) LLC size and (c) L2C size. The baseline configuration is marked in red.}
    \label{fig:sensitivity}
    % \vspace{-10pt}
\end{figure}

\subsubsection{Sensitivity to System Configurations} As shown in Fig.~\ref{fig:sensitivity}, we evaluate the performance gains when with varying off-chip bandwidth, LLC sizes {and L2C sizes}. Gaze performs well in both high- and low-bandwidth environments, and can adapt nicely to various LLC{/L2C} sizes.
The vBerti performs well under limited resources but cannot scale effectively when available resources are adequate. The over-aggressiveness of PMP leads to a extreme sharp decline when bandwidth or cache size decreases. 
% Thus, as the available resources increase, the performance gap between PMP and Gaze diminishes.
Meanwhile, the results indicate that the lightweight Gaze can effectively scale to high-bandwidth environments, such as DDR5~\cite{ddr}, and adapt to new cache technologies such as 3D V-Cache~\cite{3d_cache}.
% This is because the penalties (bandwidth contention and LLC pollution) from inaccuracy and over-aggressiveness decrease. However, even when we scale them up to levels that are challenging to achieve in reality, PMP still lags significantly behind Gaze. Meanwhile, in multi-core systems, such penalties cannot be simply ignored even with adequate resources, as over-aggressive prefetching may cause contention for shared resources (LLC and memory bandwidth), which can negatively impact other cores.


\subsubsection{Sensitivity to Gaze Configurations}
% 图13显示了Gaze在不同区域大小时在SPEC17上取得的效果，normalized to the basedline configuration。
% 从图13可以看见，较大的区域几乎总能带来性能提升，特别是在那些访问模式容易识别的工作集合上，而较小的区域很容易漏掉预取机会。平均上，使用0.5KB, 1KB, 2KB相对于使用4KB会分别带来xx,xx和xx的性能下降。这是因为使用较大的粒度能够使得一次预测容纳更多的预取请求，从而减少损失的预取机会。

% 现在大多数操作系统都支持大页面，因此，以更大粒度预测是一个可行的方向。但是，已有工作表明，适配大页面需要谨慎地对预测粒度进行切换才能带来稳定的性能提升，这大幅增加了设计复杂性。因此，我们将此留作未来工作。

% 图14显示了PHT组件在不同table size下取得的效果。通常，table size越大，所能容纳的过往经验越多，损失的预取机会就越少。在大部分工作集合上，128大小的表因为容量受限，会有较多的预取机会损失。而大于256的表只带来微弱的边际效益，这是因为256大小的表足以容纳大部分近期会被使用空间模式，增大更数倍容量去容纳的更多过往经验只有很少一部分被使用。注意，在omnetpp_s上，小的表的效果更好。这是因为该工作集展现的复杂模式不能被Gaze利用，小表减少了错误预测的数量。平均上，相较于基线设置，使用128大小的表会导致xx的性能下降，而使用512和1024大小的表则只带来xx和yy的性能提升

Fig. \ref{fig:region_pht_size}a illustrates the effect of different region sizes. The results are normalized to the baseline configuration (i.e., 4KB region). Using larger regions almost consistently yields performance improvements, particularly on workloads that are easy to follow. In contrast, using smaller regions frequently misses prefetch opportunities. On average, employing 0.5KB, 1KB, and 2KB regions results in performance degradation of 9.1\%, 4.4\%, and 1.6\%, respectively.

% Most modern operating systems support large pages~\cite{large_page}, making prediction at larger granularity a feasible direction. However, recent work has shown that a carefully-designed granularity switching strategy is required to support large pages for hardware prefetching~\cite{page_size_aware_prefetching}. This significantly increases the design complexity of spatial footprint prediction. Therefore, we leave it as future work.

\begin{figure}[tb]
    % \vspace{-10pt}
    \centering
    \includegraphics[scale=1]{figure/pht_size_and_region_size.pdf} % [width=0.45\textwidth]
    \caption{{Performance of Gaze with different configurations.}}
    \label{fig:region_pht_size}
\end{figure}

Fig. \ref{fig:region_pht_size}b presents the effect of PHT sizes. A large table can accommodate more experiences, therefore capturing more prefetching opportunities. As shown, for some workloads, the 128-entry PHT suffers from its limited capacity while 256-entry is sufficient to capture recent spatial patterns. Further increasing the capacity several-fold only brings marginal performance gains. Perversely, for workload \texttt{omnetpp}, 128-entry PHT performs the best. This is because Gaze cannot utilize its complex patterns effectively, and smaller tables reduce the number of mispredictions.
On average, compared to the baseline configuration, using a 128-entry PHT leads to a 0.6\% performance decrease, while increasing the table size to 512 and 1024 results in only 0.1\% performance gains.


% 由于当今工作负载memory footprint 的快速 grow，现代操作系统普遍利用大页面来减少地址翻译的开销，以增加TLB hit rate，并减少TLB miss的惩罚。这使得在更大区域大小上进行预取成为一个可行的方向。
% 因为Gaze工作在L1D，因此，Gaze可以在虚拟地址上使用更大的区域（我们将工作在虚拟地址下的Gaze称为vGaze）。如图17所示，我们度量了vGaze在不同区域大小的设置下的效果，normalized to the baseline configuration（4KB vGaze）。Gaze-PHT仍然被设置为4路组相联。
% 如seciii.v的分析，bwaves包含大量的spatial streaming，因此，适当增大区域能够取得不错的正面收益。但是在更多的工作负载上，使用超过4KB大小的区域会使得性能降级。我们认为这可能是因为大部分所度量的工作负载所展现的空间模式以及空间模式内部的时间关联性和4KB页面大小相匹配。因此，在缺乏OS提示下naively使用大区域并不有效。最初被访问的4KB区域的上下文并不能特征化其它4KB区域。
% Recent work has shown that，即使存在OS和ISA的支持，直接利用大页面也并总是有效，a carefully-designed granularity switching strategy is required for hardware prefetching to 获取可观的性能提升~\cite{page_size_aware_prefetching}. 在spatial-pattern-based prefetching的上下文里，这需要多个不同粒度的PHT。这和Gaze的设计相正交. Therefore, we leave it as future work.

\begin{figure}[tb]
    % \vspace{-15pt}
    \centering
    \includegraphics[scale=1]{figure/region_size_vgaze.pdf} % [width=0.45\textwidth]
    \caption{Performance of vGaze with larger region sizes.}
    \label{fig:large_region_size}
    \vspace{-10pt}
\end{figure}

{Modern operating systems (OSes) commonly use huge pages~\cite{large_page} to reduce the address translation overhead by increasing the TLB hit rate and lowering the TLB miss penalty~\cite{huge_page_1,huge_page_2}, which makes prefetching at larger region sizes a feasible direction.}
{Gaze can work at larger region sizes without specific architectural support since virtual addresses are visible at the L1D. As shown in Fig.~\ref{fig:large_region_size}, we evaluate the performance of virtual Gaze (vGaze) with different large region size settings, normalized to the baseline configuration (4KB vGaze).}
% All PHTs are still 4-way set-associative.}

{As illustrated, among the plotted traces, only \texttt{bwaves} can benefit noticeably from larger region sizes. As we have discussed in \S\ref{subsubsec:performance_analysis}, this speedup can be attributed to its streaming access. However, for most workloads, using region sizes larger than 4KB only leads to performance degradation. This suggests that most spatial patterns better align with the 4KB region size. 
Consequently, naively using larger regions is ineffective.}

{We further conduct the evaluation of accuracy and coverage. The results show that, when using small regions (less than 4KB), the accuracy remains relatively stable, but the coverage experiences a sharp decline. This reveals that smaller regions cannot effectively utilize spatial locality. In contrast, when enlarging the region size from 4KB to up to 32KB, coverage marginally grows, but the accuracy declines relatively faster. Our evaluation indicates that a region size of 4KB is suitable for Gaze.}

{Meanwhile, a recent work has shown that smartly switching the granularity based on the hint of OS page size from TLB can be effective~\cite{page_size_aware_prefetching}. Since Gaze can work in virtual address, such support is unnecessary for cross-4KB-boundary prefetching. However, multiple PHTs with different settings are required to support region size switching. It is orthogonal to the design of Gaze, and we leave it as future work.}

% Effect of the size of Berti tables. Figure 22 shows
% the effect of the size of the Berti tables (history table,
% table of deltas, and the number of deltas) on speedup.
% Decreasing the size of the table of deltas by a quarter
% degrades performance by 12.1%, whereas decreasing the
% number of deltas by a quarter reduces performance by 1.2%.
% Also, doubling/quadrupling the size of the tables provides
% a marginal performance gain. CactuBSSN is one outlier
% where increasing the table sizes to 1024 entries with 1024
% sets improve performance by 22%.

% \begin{figure}[htb]
%     \vspace{-3pt}
%     \centering
%     \includegraphics[scale=1]{figure/pht_size.pdf} % [width=0.45\textwidth]
%     \caption{{Speedup achieved by PHT with different table sizes.}}
%     \label{fig:pht_size}
%     % \vspace{-12pt}
% \end{figure}
% In a word, Gaze has comparable hardware overhead to the state-of-the-art L1D prefetcher, PMP, and achieves the highest performance among all evaluated prefetchers. Therefore, Gaze is well-suited to operate solely in either of these two levels.

% \textbf{Varying} In principle, prefetchers working at L1D can eliminate more misses since the full access sequences can be observed. However, surprisingly, all evaluated prefetchers achieve higher coverage (15.3\% higher on average) and almost the same speedup when deployed solely at L2C. We find that, compared to L1D, L2C typically has more MSHR entries, allowing more load and prefetch requests to be issued simultaneously. And, when working at L1D, prefetching is constrained by the limited MSHR entries, resulting in fewer successfully-issued prefetch requests despite the full access sequence can be observed. One way is to deploy Gaze at L1D, but prefetch all blocks into L2C. In this manner, prefetched blocks do not return to L1D, thus not consuming L1D MSHR entries. This makes full use of the abundant resources in L2C and the full access sequences in L1D, further enhancing the performance of Gaze by 1.7\%. 
% \subsubsection{Effect of OoO}


==> texfile/8_relat.tex <==
\section{Other Related Work}
\label{sec:relatedwork}
\textbf{Prefetching} has been extensively studied over decades.
% Recent years, due to the increasing emergence of memory-intensive applications, architects have proposed numerous data prefetchers to overcome the slowdown of DRAM scaling.
\textit{Delta-correlated spatial prefetchers} including BOP~\cite{BOP}, SPP~\cite{SPP}, and Berti~\cite{Berti} try to predict future deltas. BOP records the scores of every delta and selects the one with the highest score. Berti works in a per-PC view and further takes into account the fetch latency to serve a timely and accurate prefetching. SPP and IPCP-CPLX~\cite{IPCP} use signature-based methods to recognize complex strides.
\textit{Temporal prefetchers}~\cite{Domino,Triage,MISB,STeMS,Markov,ISB,STMS,GHB} try to extract temporal similarity of access patterns. They are proficient at recognizing irregular access patterns such as pointer-based access. However, they suffer from the huge storage overhead since the demand sequences are stored.
Some prefetchers apply \textit{machine learning} in hardware prefetching~\cite{Pythia,ML_Pref_1,ML_Pref_2,ML_Pref_3}, where Pythia~\cite{Pythia}, a reinforcement learning-based hardware prefetcher, achieves both high performance and acceptable hardware complexity.
\textit{Pre-computation}~\cite{pre_exec_1,pre_exec_2,pre_exec_3,pre_exec_4,pre_exec_5,pre_exec_6,pre_exec_7,pre_exec_8} issues prefetch requests through pre-executing program code. They can generate highly-accurate prefetches without the need for access patterns. However, pre-executing dramatically increases the hardware complexity.
\textit{Cache level prediction}~\cite{TLP,Hermes,CLP_1,CLP_2,CLP_3,CLP_4} hides the on-chip cache hierarchy latency by predicting which level a load might hit and fetch the data directly. Hermes~\cite{Hermes} uses a perceptron-based mechanism to predict which demands might go off-chip.

{\bf Spatial footprint prediction} is also leveraged in several DRAM cache techniques~\cite{FootprintCache_1, FootprintCache_2, FootprintCache_3, FootprintCache_4} to harness the advantages of both cacheline- and page-based designs. They manage data at a coarse granularity to avoid infeasible large tag space, while fetching only the blocks that will be used during the residency of the page to overcome the over-fetching problem.


==> texfile/9_conc.tex <==
\section{Conclusion}
% \vspace{-5pt}
\label{sec:conclusion}
In this paper, we highlight that the underlying limitation of spatial-pattern-based prefetching is its pattern characterization scheme.
To this end, we propose Gaze, a lightweight and efficient hardware prefetcher that Gaze skillfully applies the temporal correlation of the first several spatial accesses to characterize patterns, which makes it capable of predicting more accurately with low hardware cost.
% Concurrently, we employ a two-stage aggressiveness promotion strategy to mitigate the risks associated with employing prefetch patterns that indicate to fetch the entire regions.
Concurrently, Gaze introduces a dedicated two-stage approach to mitigate the over-prefetching problem that often occurs in spatial streaming.
In our evaluation, Gaze adapts well to both low-bandwidth and high-bandwidth environments and exhibits excellent performance in multi-core simulations. Gaze outperforms PMP and vBerti by 5.7\% and 5.4\% at single-core and by 11.4\% and 8.8\% at eight-core.

% Meanwhile, we observe that employing the prefetch pattern which indicates to fetch the whole spatial region has a extremely high risk. Therefore, we further enhance Gaze with a two-stage aggressiveness promotion strategy for this to balance between the desire for the entire region and its possible massive negative effects.
% In this paper, we note that the temporal correlation exhibited within a spatial pattern can efficiently characterize different spatial access behaviors. To this end, we propose Gaze, a simple and efficient hardware spatial prefetcher that skillfully applies the temporal correlation of the first several spatial accesses to make exact predictions. Meanwhile, we observe that employing the prefetch pattern which indicates to fetch the whole spatial region has a extremely high risk. Therefore, we further enhance Gaze with a two-stage aggressiveness promotion strategy for this to balance between the desire for the entire region and its possible massive negative effects.

% Our comprehensive and diverse set of experiments shows that Gaze can effectively enhance the performance across a wider range of scenarios. Specifically, Gaze improves performance by xx\% and xx\% at single-core, xx\% and xx\% at eight-core, compared to most recent low-cost solutions Berti and PMP.
